Model-Protected Multi-Task Learning

Multi-task learning (MTL) refers to the paradigm of learning multiple related tasks together. In contrast, in single-task learning (STL) each individual task is learned independently. MTL often leads to better trained models because they can leverage the commonalities among related tasks. However, because MTL algorithms can ``leak" information from different models across different tasks, MTL poses a potential security risk. Specifically, an adversary may participate in the MTL process through one task and thereby acquire the model information for another task. The previously proposed privacy-preserving MTL methods protect data instances rather than models, and some of them may underperform in comparison with STL methods. In this paper, we propose a privacy-preserving MTL framework to prevent information from each model leaking to other models based on a perturbation of the covariance matrix of the model matrix. We study two popular MTL approaches for instantiation, namely, learning the low-rank and group-sparse patterns of the model matrix. Our algorithms can be guaranteed not to underperform compared with STL methods. We build our methods based upon tools for differential privacy, and privacy guarantees, utility bounds are provided, and heterogeneous privacy budgets are considered. The experiments demonstrate that our algorithms outperform the baseline methods constructed by existing privacy-preserving MTL methods on the proposed model-protection problem.

==> abstract_and_intro.tex <==
%!TEX root = MultitaskDP.tex
%\IEEEtitleabstractindextext{%


%\begin{abstract}
%Multi-task learning (MTL) refers to the paradigm of learning multiple related tasks together. {By contrast, single-task learning (STL) refers to the paradigm of learning each individual task independently.} MTL often leads to better trained models because they can leverage the commonalities among related tasks.
%%In the last decade, MTL has been successfully applied in many application areas, including computer vision, natural language processing and healthcare.
%However, because MTL algorithms will ``transmit" information {of models} across different tasks, there is a potential security risk. {For example, in the area of adversarial attack, model leakage could escalate black-box attacks into white-box attacks. In health informatics, leaking a personalized model means leaking reasons of diseases of a patient.} Earlier privacy-preserving MTL methods protect data instances { rather than models}, some of which may underperform STL methods. In this paper, we propose a private MTL framework {to protect the information of each model from leaking to other models} based on a perturbation of the covariance matrix of the model matrix, and we study two popular MTL approaches for instantiation: the MTL approaches for learning the low-rank and group-sparse pattern of the model matrix. Our methods are built upon the tools of differential privacy. {Privacy guarantees and utility bounds are provided. We are the first to provide utility analysis for differentially private MTL algorithms that allows heterogeneous tasks. Heterogeneous privacy budgets are considered, and utility analysis for budget allocation is provided. Our algorithms can be guaranteed to not underperform STL methods. Experiments demonstrate that our algorithms outperform existing privacy-preserving MTL methods.}
%%The privacy-accuracy trade-offs offered by each approach are evaluated. Our methods protect both the data and the model parameters of each task from potential attack from other related tasks. The effectiveness of our framework is demonstrated on both synthetic and real-world datasets. Our methods outperform existing privacy-preserving MTL methods, especially when one has high demand for privacy.
%\end{abstract}


%\begin{abstract}
%Multi-task learning (MTL) refers to the paradigm of learning multiple related tasks together. {By contrast, single-task learning (STL) refers to the paradigm of learning each individual task independently.} MTL often leads to better trained models because they can leverage the commonalities among related tasks.
%However, because MTL algorithms will ``transmit" information {on different models} across different tasks, MTL poses a potential security risk. {Specifically, an adversary may participate in the MTL process through a participating task, thereby acquiring the model information for another task.} Previously proposed privacy-preserving MTL methods protect data instances { rather than models}, and some of them may underperform in comparison with STL methods. In this paper, we propose a privacy-preserving MTL framework {to prevent the information on each model from leaking to other models} based on a perturbation of the covariance matrix of the model matrix, and we study two popular MTL approaches for instantiation, namely, MTL approaches for learning the low-rank and group-sparse patterns of the model matrix. Our methods are built upon tools for differential privacy. {Privacy guarantees and utility bounds are provided. We are the first to present utility analyses for differentially private MTL algorithms that allow heterogeneous tasks. Heterogeneous privacy budgets are considered, and utility analyses for budget allocation are presented. Our algorithms can be guaranteed not to underperform in comparison with STL methods. Experiments demonstrate that our algorithms outperform existing privacy-preserving MTL methods on the proposed model-protection problem.}
%\end{abstract}
%
%% Note that keywords are not normally used for peerreview papers.
%\begin{IEEEkeywords}
%Multi-Task Learning, Model Protection, Differential Privacy, Covariance Matrix, Low-Rank Subspace Learning.
%\end{IEEEkeywords}
%}

 % make the title area
%\maketitle

% To allow for easy dual compilation without having to reenter the
% abstract/keywords data, the \IEEEtitleabstractindextext text will
% not be used in maketitle, but will appear (i.e., to be "transported")
% here as \IEEEdisplaynontitleabstractindextext when the compsoc
% or transmag modes are not selected <OR> if conference mode is selected
% - because all conference papers position the abstract like regular
% papers do.
%\IEEEdisplaynontitleabstractindextext
% \IEEEdisplaynontitleabstractindextext has no effect when using
% compsoc or transmag under a non-conference mode.



% For peer review papers, you can put extra information on the cover
% page as needed:
% \ifCLASSOPTIONpeerreview
% \begin{center} \bfseries EDICS Category: 3-BBND \end{center}
% \fi
%
% For peerreview papers, this IEEEtran command inserts a page break and
% creates the second title. It will be ignored for other modes.
\IEEEpeerreviewmaketitle



%\IEEEraisesectionheading{}

\section{Introduction}\label{sec:introduction}


%\section{Introduction}

\IEEEPARstart{M}{ulti-task learning} (MTL)~\citep{caruana1997multitask} refers to the paradigm of learning multiple related tasks together. {By contrast, single-task learning (STL) refers to the paradigm of learning each individual task independently.} MTL often leads to better trained models because the commonalities among related tasks may assist in the learning process for each specific task. For example, the capability of an infant to recognize a cat might help in the development of his/her capability to recognize a dog. In recent years, MTL has received considerable interest in a broad range of application areas, including computer vision~\citep{li2010probabilistic,zhang2012robust}, natural language processing~\citep{almeida2013fast} and health informatics~\citep{sun2015linkage,wang2014exploring}. {\color{blue}The key to MTL is to relate the tasks via a shared representation, which, in turn, benefits the tasks to be learned. Each possible shared representation encodes certain assumptions regarding the task relatedness.
A typical/main-stream assumption is that the tasks share a latent low-rank subspace, as stated by \citet{zhang2017survey} in their survey on MTL, and also by \citet{su2018multi} and \citet{gu2016low}; see, e.g.,~\citet{ando2005framework},~\citet{chen2009convex},~\citet{xu2012conditional},~\citet{han2016multi}, and~\citet{zhen2018multi}.}
 
 
 
 
Because MTL approaches explore and leverage the commonalities among related tasks within the learning process, either explicitly or implicitly, they pose a potential security risk.
Specifically, an adversary may participate in the MTL process through a participating task, thereby acquiring the model information for another task. {\color{blue}A predictive model may identify a causality between inputs and outputs of a system. Knowledge of the causality makes it possible or easier for an adversary to change an input of the system to trigger an irrational and even harmful output, which can be regarded as a  \emph{generalized adversarial attack}. The aforementioned system could be not only a predictive system for traffic-sign recognition or face identification, as studied by recent adversarial-attack approaches~\citep{szegedy2013intriguing,moosavi2016deepfool,kurakin2016adversarial,zantedeschi2017efficient,papernot2016practical,papernot2016transferability,mopuri2017fast}, but also a real human body. For example, we consider \emph{personalized predictive modeling}~\citep{ng2015personalized,zhang2014towards}, which has become a fundamental methodology in health informatics. In this type of modeling, a custom-made model is built for each patient. In modern health informatics, such a model may contain disease conditions/causes of a patient, e.g., what food can induce allergy of a patient. Therefore, if such information is leaked to an adversary, s/he will use the information to deliberately put the food in the meal of the patient to trigger allergy, which is disastrous.}

%Such information is a different type of privacy from that of any single data record, and also requires protection. However, the joint training of personalized models may allow such causes of disease to be leaked to an adversary whose model is also participating in the joint training.
 

%Fig.~\ref{fig:privacy_leakage} provides illustrations for model leakage and model protection under a specific MTL approach capturing the low rank pattern of the model matrix (Notations are defined in the next section and in Algorithm \ref{alg:MP-MTL-LR}).


%\begin{figure}[!t]\small
%\centering
%\subfigure[Before MTL]{\includegraphics[width=1.1in]{lowrank_before}} %diffk_simu_nmseg_1
%\subfigure[After MTL with model leakage]{\includegraphics[width=1.1in]{lowrank_after}} %diffk_simu_aauc_1
%\subfigure[After MTL with model protection]{\includegraphics[width=1.1in]{lowrank_after_add_noise}} %diffk_simu_aauc_1
%\caption{Examples of model leakage and model protection, showing models before and after MTL, where columns are for tasks, rows are for features. The 10-th task is the anomaly task that requires privacy protection. In (a), the matrix denoted by $\W^{(0)}$ is firstly generated by i.i.d. uniform distribution $\mathcal{U}(0,1)$. Then the last column is multiplied by $100$. We then run Algorithm \ref{alg:MP-MTL-LR}, taking $m=10,d=5,T=1,\epsilon_1 = \epsilon = 0.1, \delta = 0, K = 100\sqrt{5}, \lambda = 50$. $\eta$ is irrelevant since $T=1$. The noise matrix $\E$ has not been added in (b) and has been added in (c). (a) shows $\W^{(0)}$; (b) and (c) show $\widehat{\W}^{(1)}$ under their respective settings. Columns are divided by their respective $\ell_2$ norms when plotting in pictures. In (b), the 10-th task results in significantly changes in the parameters of other models, especially for the first and the last features. In (c), the changes from the 10-th task are not significant. Meanwhile, the second feature is shared by most tasks as should be.}\label{fig:privacy_leakage}
%\end{figure}

%\begin{figure}[!t]\small
%\centering
%\subfigure[Low rank - Before]{\includegraphics[width=1.7in]{lowrank_before}} %diffk_simu_nmseg_1
%\subfigure[Low rank - After]{\includegraphics[width=1.7in]{lowrank_after}} %diffk_simu_aauc_1
%\subfigure[Group sparse - Before]{\includegraphics[width=1.7in]{groupsparse_before}} %diffk_simu_nmseg_2
%\subfigure[Group sparse - After]{\includegraphics[width=1.7in]{groupsparse_after}} %diffk_simu_aauc_2
%\caption{Examples of model leakage, showing absolute values of parameters before and after proximal operators, where columns are for tasks, rows are for features. (a) and (b) are examples for proximal operator with trace norm (equation \ref{eq:proximal_op_LR}), (c) and (d) are examples for proximal operator with group $\ell_1$ norm (equation \ref{eq:proximal_op_GS}). For both cases, the 10-th task is the new task which results in significantly change in the parameters of other models after the joint learning.}\label{fig:privacy_leakage}
%\end{figure}



%For example, risk prediction is a fundamental problem in modern health informatics. Various predictive models have been developed for the early detection of chronic disease based on patients' historical records~\citep{bayati2015low,wang2014exploring,wu2010prediction}. Due to the complexity of chronic diseases, patients are usually associated with one or more chronic morbidities. The studies of~\citet{bayati2015low} and~\citet{wang2014exploring} demonstrate that using MTL approaches for the joint prediction of the onset risk of multiple related chronic conditions (e.g., heart failure, chronic obstructive pulmonary disease, and diabetes) may achieve better performance compared with predicting each individual disease separately. In this case, if the predictor information of one disease is leaked, the attacker may also obtain information about the predictors for other diseases. This could prove disastrous, as the attacker will know all potential chronic conditions for the patients. {Specifically, consider the case of two hospitals: hospital A is in charge of a disease containing a large amount of personal information that may influence one's reputation or career, and so demands high privacy; hospital B is in charge of another disease containing inconsequential information, and then demands low privacy. Although hospital A may acquire more protection for its data, if Bob's demographic data (or other simple data such as blood pressure, heart rate, diet, sports, etc.) exists in both hospitals, and both hospitals participate into some MTL procedure, then a hacker may only need to hack the data and the predictive model of hospital B due to insufficient protection to inference the model of hospital A due to model leakage. As such, because some of Bob's data are already in hospital B, the hacker can easily predict Bob's condition of the disease which is in the charge of hospital A, and go against Bob.} Therefore, it is necessary to develop a secure training strategy for MTL approaches such that information leaks from one task will not affect the predictors for other tasks. The requirement to ensure the security of models/predictors from such leakage caused by joint learning is also considered by~\citet{shokri2015privacy} and~\citet{liu2015fast}.

Because of the concerns discussed above, it is necessary to develop a secure training strategy for MTL approaches to prevent information on each model from leaking to other models. In this paper, we propose model-protected multi-task learning (MP-MTL), which enables the joint learning of multiple related tasks while simultaneously preventing leakage of the models for each task. We use tools offered by \emph{differential privacy}~\citep{dwork2014algorithmic}, which provides a strong, cryptographically motivated definition of privacy based on rigorous mathematical theory and has recently received significant research attention due to its robustness to known attacks~\citep{chaudhuri2011differentially,ganta2008composition}. This scheme is useful when one wishes to prevent potential attackers from acquiring information on any element of the input dataset based on a change in the output distribution.


%To overcome these shortcomings, in this paper, we propose model-protected multi-task learning (MP-MTL), which enables the joint learning of multiple related tasks while simultaneously preventing leakage of the models for each task.



%under a rigorous theoretical guarantee of differential privacy.

%For the measure of model leakage, we adopt the tools offered by differential privacy~\citep{dwork2014algorithmic}, which provides a strong, cryptographically motivated definition of privacy with rigorous mathematical theory and has recently received a significant amount of research attention for its robustness to known attacks~\citep{chaudhuri2011differentially,ganta2008composition}, where one wishes to avoid potential attackers acquiring the information of any element of the input dataset based on a change in the output distribution.

%To the best of our knowledge, most differentially private learning algorithms focus on ensuring the security of data instances, which include differentially private versions of linear and logistic regression~\citep{chaudhuri2008privacy,zhang2012functional}, support vector machines~\citep{rubinstein2009learning}, risk minimization~\citep{chaudhuri2011differentially,wainwright2012privacy}, boosting~\citep{dwork2010boosting}, principal component analysis~\citep{chaudhuri2013near,dwork2014analyze,jiang2016wishart,imtiaz2016symmetric} and deep learning~\citep{shokri2015privacy,abadi2016deep}. However, few privacy-preserving multi-task learning approaches~\citep{mathew2012distributed,baytas2016asynchronous,pathak2010multiparty,shokri2015privacy,gupta2016differentially} have been proposed. Such methods only protect the data instances instead of the models/predictors.


\begin{figure}[t!]
\centering
\includegraphics[width=3.5in]{system1}
\caption{{Model-Protected Multi-Task Learning framework. The solution process is a recursive two-step procedure. The first step is a decoupled learning procedure in which the model parameters for each task are estimated independently using the pre-computed shared information among tasks. The second step is a centralized transfer procedure in which the information shared among tasks is extracted for distribution to each task for the decoupled learning procedure in the next step. The shared information is extracted from the tasks' covariance matrix, into which Wishart noise is introduced to ensure the security of the models.}}\label{fig:framework}
\end{figure}


%For our privacy measure, we use a definition in~\citep{dwork2006our}, where a measure of quantifying the privacy-risk associated with computing functions of sensitive data is proposed. Such $(\epsilon,\delta)$-differential privacy model is a strong, cryptographically-motivated definition of privacy that has recently received a significant amount of research attention for its robustness to known attacks~\citep{chaudhuri2011differentially}\cite{ganta2008composition}.

%Algorithms satisfying $(\epsilon,\delta)$-differential privacy are randomized; the output is a random variable whose distribution is conditioned on the data set. A statistical procedure satisfies $(\epsilon,\delta)$-differential privacy if changing a single data point does not shift the output distribution by too much.

Without loss of generality, our MP-MTL method is designed based on linear multi-task models~\citep{ji2009accelerated,liu2009multi}, in which we assume that the model parameters are learned by minimizing an objective that combines an average empirical prediction loss and a regularization term. The regularization term captures the commonalities among the different tasks and couples their model parameters. The solution process for this type of MTL method can be viewed as a recursive two-step procedure. The first step is a decoupled learning procedure in which the model parameters of each task are estimated independently using some pre-computed shared information among tasks. The second step is a centralized transfer procedure in which some of the information shared among tasks is extracted for distribution to each task for the decoupled learning procedure in the next step. Our MP-MTL mechanism protects the models by adding perturbations during this second step. {Note that we assume a curator that collects models for joint learning but never needs to collect task data.} We develop a rigorous mathematical definition of the MP-MTL problem and propose an algorithmic framework to obtain the solution. We add perturbations to the covariance matrix of the parameter matrix because the tasks' covariance matrix is widely used as a fundamental ingredient from which to extract useful knowledge to share among tasks~\citep{liu2009multi, zhang2010convex, ji2009accelerated,argyriou2007multi,zhou2011clustered,sun2015linkage}, {\color{blue}which is the key observation that enables the proposed framework.} The usage of the perturbed covariance matrix depends on the specific MTL method applied. Consequently, our technique can cover a wide range of MTL algorithms and {\color{blue}is generally applicable for many optimization schemes, such as proximal gradient methods~\citep{ji2009accelerated,liu2009multi}, alternating methods~\citep{argyriou2007multi} and Frank-Wolfe methods~\citep{jaggi2013revisiting}}. Wishart noise is introduced into the covariance matrix to ensure the security of the models. Fig. \ref{fig:framework} illustrates the key ideas of the main framework. {\color{blue}Note that although our framework is designed based on linear models, it can be extended to non-linear models. Typically, consider designing a deep neural network for each task. The network structures between tasks are identical, while the parameters of networks are different between tasks. Then for each layer of the networks, a covariance matrix can be computed using vectorized parameters of tasks. Then our approach can be extended to such a setting, designing perturbations for these covariance matrices. }



We further develop two concrete approaches as instantiations of our framework, each of which transforms an existing MTL algorithm into a private version. Specifically, we consider two popular types of basic MTL models: 1) a model that learns a low-rank subspace by means of a trace norm penalty~\citep{ji2009accelerated} and 2) a model that performs shared feature selection by means of a group-$\ell_1$ ($\ell_{2,1}$ norm) penalty~\citep{liu2009multi}. {\color{blue}In both cases, we instantiate our framework by approximating \emph{proximal gradient descent methods} presented by~\citet{ji2009accelerated} and~\citet{liu2009multi}, respectively. The covariance matrix is used to build a linear transform matrix with which to project the models into new feature subspaces, among which the most useful subspaces are selected. The projection matrix is related to the generalized inverse of the singular value matrix (or the diagonal matrix) of the perturbed covariance matrix for the instantiation with a trace norm penalty (or the instantiation with a group-$\ell_1$ penalty). Wishart noise is positive definite and thus can only render the perturbed covariance matrix ``larger'' and render the generalized inverse ``smaller''. Consequently, the projection matrix tends to be an identity matrix under high noise level, which shares no information between models but keeps the models intact. This means that our algorithms will not underperform in comparison with STL methods under high noise level, hence participation in the joint learning process will have no negative effect on the training of any task model. Approximating the proximal operators with Wishart noise makes it possible for added noises to destroy the covariance matrix without destroying the projected models, which is a key observation that enables the proposed instantiate algorithms.}

Privacy guarantees are provided. Utility analyses are also presented for both convex and strongly convex prediction loss functions and for both the basic and accelerated proximal-gradient methods. Furthermore, heterogeneous privacy budgets are considered for different iterations of our algorithms, and a utility analysis for privacy-budget allocation is presented. We also validate the effectiveness of our approach on benchmark and real-world datasets. 

{\color{blue}Our proposed MP-MTL algorithms fall into a larger scope of differentially private MTL algorithms (i.e., MTL algorithms with randomness added using tools of differential privacy). Within this scope, to the best of our knowledge, we are the first to present a utility analysis for heterogeneous tasks. By contrast, the distributed tasks studied by~\citet{pathak2010multiparty} are homogeneous; i.e., the coding procedures for both features and targets are the same for different tasks. We are also the first to provide privacy guarantees for heterogeneous tasks and for loss functions that do not have closed-form solutions (e.g., the logistic loss).}



%The utility results under the best privacy-budget allocation strategies are summarized in Table \ref{tab:utility_results} (the notations used in the table are defined in the next section).} 

{\color{blue}Since our method are the first to address the model-protected problem in MTL setting, we construct baseline MP-MTL methods for comparison by exploiting existing privacy-preserving MTL methods which are referred to as instance-protected multi-task learning (IP-MTL) methods because they only protect the security of data instances rather than that of models. The IP-MTL methods are transformed into their respective MP-MTL methods by directly enforcing \emph{group privacy}~\citep{dwork2014algorithmic} of the entire dataset coming from a single learning task. The experimental results demonstrate that our proposed algorithms outperform the constructed baseline MP-MTL methods.}

%In addition, we analyze the difference between our MP-MTL scheme and the existing privacy-preserving MTL strategies, which ensure the security of data instances.


%Since existing privacy-preserving MTL methods only protect single data instances, they are transformed into methods that can protect task models using our theoretical results. 






%\setlength{\tabcolsep}{1pt}
%\begin{table}[htbp]\small
%  \centering
%  %\renewcommand{\multirowsetup}{\centering}
%  \begin{tabular}{c|c|c|c|c}
%     \hline
%   &\multicolumn{2}{c|}{No acceleration}& \multicolumn{2}{c}{Accelerated}\\
%   \hline
%   &Convex   &Strong convex &Convex   &Strong convex\\
%   \hline
%   Low rank& $\mathcal{O}((\frac{d\log(d)}{\sqrt{m}\epsilon})^{\frac{2}{5}})$ & $\mathcal{O}((\frac{d\log(d)}{\sqrt{m}\epsilon})^{\frac{1}{2}})$ & $\mathcal{O}((\frac{d\log(d)}{\sqrt{m}\epsilon})^{\frac{4}{9}})$ & $\mathcal{O}((\frac{d\log(d)}{\sqrt{m}\epsilon}))$\\
%   \hline
%   Group sparse&$\mathcal{O}((\frac{\log(d)}{{m}\epsilon})^{\frac{2}{5}})$ & $\mathcal{O}((\frac{\log(d)}{{m}\epsilon})^{\frac{1}{2}})$ & $\mathcal{O}((\frac{\log(d)}{{m}\epsilon})^{\frac{4}{9}})$ & $\mathcal{O}((\frac{\log(d)}{{m}\epsilon}))$\\
%   \hline
%  \end{tabular}
%  \caption{Utility results.}\label{tab:utility_results}
%\end{table}

%\setlength{\tabcolsep}{2pt}
%\begin{table}[htbp]\small
%  \centering
%  \renewcommand{\multirowsetup}{\centering}
%    \caption{Utility results.}\label{tab:utility_results}
%  \begin{tabular}{c|c|c|c}
%  \hline
%     \hline
%     & &Low rank& Group sparse\\
%     \hline
%     \multirow{2}{*}{No acceleration}&Convex& $\mathcal{O}((\frac{d\log(d)}{\sqrt{m}\epsilon})^{\frac{2}{5}})$ &$\mathcal{O}((\frac{\log(d)}{{m}\epsilon})^{\frac{2}{5}})$ \\
%   \cline{2-4}
%   &Strong convex&$\mathcal{O}((\frac{d\log(d)}{\sqrt{m}\epsilon})^{\frac{1}{2}})$ &$\mathcal{O}((\frac{\log(d)}{{m}\epsilon})^{\frac{1}{2}})$ \\
%    \hline
%    \multirow{2}{*}{Accelerated}&Convex&$\mathcal{O}((\frac{d\log(d)}{\sqrt{m}\epsilon})^{\frac{4}{9}})$  & $\mathcal{O}((\frac{\log(d)}{{m}\epsilon})^{\frac{4}{9}})$\\
%    \cline{2-4}
%    &Strong convex&$\mathcal{O}(\frac{d\log(d)}{\sqrt{m}\epsilon})$&$\mathcal{O}(\frac{\log(d)}{{m}\epsilon})$\\
%   \hline
%   \hline
%  \end{tabular}
%\end{table}



%where we assume there is a low-rank structure on the model parameter matrix and the perturbation is added on its spectrum. This is because getting the spectrum is a necessary step when we adopt trace norm as the regularizer, which is a popular choice for MTL methods to control the model complexity.
%In this way, we can get a ``secure" estimate of model parameters at each iteration and thus make the final solution differentially private. We also validate the effectiveness of our approach on benchmark and real world data sets.

The contributions of this paper are highlighted as follows.
\begin{itemize}
\item {We are the first to propose and address the model-protection problem in MTL setting.}
\item We develop a general algorithmic framework to solve the MP-MTL problem to obtain secure estimates of the model parameters. We derive concrete instantiations of our algorithmic framework for two popular types of MTL models, namely, models that learn the low-rank and group-sparse patterns of the model matrix. {\color{blue}By approximating proximal operators with Wishart noise}, it can be guaranteed that our algorithms will not underperform in comparison with STL methods under high noise level.
\item Privacy guarantees are provided. Utility analyses are also presented for both convex and strongly convex prediction loss functions and for both the basic and accelerated proximal-gradient methods. Heterogeneous privacy budgets are considered for different iterations of our algorithms, and a utility analysis for privacy-budget allocation is presented.  
\item {\color{blue}Within the larger scope of differentially private MTL algorithms, to the best of our knowledge, we are the first to provide privacy guarantees for heterogeneous tasks and for loss functions that do not have closed-form solutions. We are also the first to present utility analyses for heterogeneous tasks and the first to present allocation strategies for heterogeneous privacy budgets.}
\item {\color{blue}For comparison, we construct baseline MP-MTL methods using IP-MTL methods (i.e., existing privacy-preserving MTL methods). Experiments demonstrate that our proposed algorithms significantly outperform them.}
\end{itemize}


The remainder of this paper is organized as follows. {\color{blue}Section \ref{sec:related_work} discusses related works and definitions of differential privacy.} Section \ref{sec:pre} introduces the background on MTL problems and the definition of the proposed model-protection problem. The algorithmic framework and concrete instantiations of the proposed MP-MTL method are presented in Section \ref{sec:method}, {along with the analyses of utility and privacy-budget allocation}. Section \ref{sec:exp} presents an empirical evaluation of the proposed approaches, followed by the conclusions in Section \ref{sec:conclusion}. 

\section{Related Works}\label{sec:related_work}

\subsection{Privacy-preserving MTL approaches}

Few privacy-preserving MTL approaches have been proposed to date~\citep{mathew2012distributed,baytas2016asynchronous,pathak2010multiparty,shokri2015privacy,gupta2016differentially}. Moreover, such approaches protect only the security of data instances rather than that of models. A typical focus of research is distributed learning~\citep{mathew2012distributed,baytas2016asynchronous}, in which the datasets for different tasks are distributively located. The local task models are trained independently using their own datasets before being aggregated and injected with useful knowledge shared across tasks. Such a procedure mitigates the privacy problem by updating each local model independently. However, these methods do not provide theoretical guarantees of privacy.


 
\citet{pathak2010multiparty} proposed a differentially private aggregation (DP-AGGR) method in a distributed learning scheme with privacy guarantees.
% \citet{pathak2010multiparty} proposed a differentially private aggregation (DP-AGGR) method in a distributed learning scheme with privacy guarantees using tools offered by \emph{differential privacy}~\citep{dwork2014algorithmic}, which provides a strong, cryptographically motivated definition of privacy based on rigorous mathematical theory and has recently received significant research attention due to its robustness to known attacks~\citep{chaudhuri2011differentially,ganta2008composition}. This scheme is useful when one wishes to prevent potential attackers from acquiring information on any element of the input dataset based on a change in the output distribution.
%%%Editor - Please ensure that the intended meaning has been maintained
%%%in the above edit.
\citet{pathak2010multiparty} first trained local models distributively and then averaged the models of the tasks before adding noise based on the output perturbation method of~\citep{dwork2006calibrating}. The final solution for each task is the averaged model. However, because only averaging is performed in this method, it has a limited ability to cover {more complicated relations among tasks, such as low-rank~\citep{ando2005framework}, group-sparse~\citep{turlach2005simultaneous}, clustered~\citep{gu2009learning} or graph-based~\citep{zhang2010convex} task structures}. 

\citet{gupta2016differentially} proposed a differentially private multi-task relationship learning (DP-MTRL) method to transform the multi-task relationship learning proposed by~\citet{zhang2010convex} into a differentially private version, in which the output perturbation method is also adopted. {However, their method requires a closed-form solution (obtained by minimizing the least-square loss function) to achieve a theoretical privacy guarantee; thus, it cannot guarantee the privacy for methods like logistic regression who needs iterative optimization procedures}. Moreover, on their synthetic datasets, their privacy-preserving MTL methods underperformed comparing with non-private STL methods (which can guarantee optimal privacy against the leakage of information across tasks), which suggests that there is no reason to use their proposed methods. {In addition, they did not study the additional privacy leakage due to the iterative nature of their algorithm (see~\citet{kairouz2017composition}), and they did not study the utility bound for their method}. 

The approaches of both~\citet{pathak2010multiparty} and~\citet{gupta2016differentially} protect a single data instance instead of the model of each task, and they involve adding noise directly to the models, which is unnecessary for avoiding the leakage of information across tasks and may jeopardize the utility of the algorithms. 

{\color{blue}

\subsection{Related Works of Differential Privacy}\label{subsec:related_def}

Several related definitions of privacy are listed as follows.

\noindent\textbf{\emph{\underline{Joint differential privacy}}}. It is proposed by \citet{kearns2015robust} and \citet{kearns2014mechanism} in the setting of game theory to guarantee that for each player, the mechanism output for other players does not reveal much input information of the player. Besides detailed concepts of game theory, such as player type, this definition can be regarded identical to the privacy constraint used in our proposed MP-MTL algorithms. 

\noindent\textbf{\emph{\underline{One-analyst-to-many-analyst privacy}}}. It is proposed by \citet{hsu2013differential} in the setting of querying databases to protect the privacy of all the queries of one analyst from other analysts. They also proposed a related privacy called \emph{one-query-to-many-analyst privacy}. Both definitions of privacy can be regarded identical to the privacy constraints used in our proposed MP-MTL and our defined IP-MTL algorithms, respectively, besides detailed concepts of database query. 

Roughly speaking, the above approaches and this paper adopt the same privacy constraint, but work on different specific fields. We would like to clarify that our contribution is not to propose a new type of privacy constraint, but is to raise the privacy problem in MTL setting and propose a method to handle the problem.

\noindent\textbf{\emph{\underline{Differential privacy for streams}}}. It is proposed by \citet{chan2011private} and \citet{dwork2010differential} to handle continual/iterative observation. Since machine learning algorithms are iterative in general, this paper also involves the concept of iteration in the definitions of MP-MTL and IP-MTL algorithms, which is not claimed as one of our contribution, because it just aims to directly use composition theorems of differential privacy to bound the total privacy-budgets.

%for both the iterative algorithms. Usually, differentially private machine learning approaches just consider their iterative processes in their proofs for privacy guarantees (see, e.g., \citet{talwar2015nearly}, \citet{wang2017differentially}, and \citet{zhang2017efficient}), while this paper directly involves the concept of iteration in the definitions. 

\noindent\textbf{\emph{\underline{Local private learning algorithms}}}. The definition is proposed by \citet{kasiviswanathan2011can} to characterize that each individual’s data are added independent randomness before being processed. Such algorithms are also referred to as input perturbation. Its idea can be adopted for possible solutions to the MP-MTL problem. For example, independent randomness can be added to the model of each task. Both DP-MTRL and DP-AGGR can be regarded as such examples, although they protects data instances rather than models. Since local private learning algorithms have their limitations (e.g., may require exponentially more data than general private algorithms do~\citep{kasiviswanathan2011can}), we did not adopt the idea to construct our MP-MTL method.

\noindent\textbf{\emph{\underline{Secure multi-party computation (SMC)}}}. In Section 1, one may observe that we assume the use of a trusted curator that collects the task models; this assumption will raise privacy concerns in settings in which the curator is untrusted. Such concerns are related to the demand for SMC~\citep{pathak2010multiparty,goldreich1998secure}, {the purpose of which is to avoid the leakage of data instances to the curator}. Our extended framework considering SMC is presented in the supplementary material.

Besides the above related definitions, the sample-aggregate framework proposed by \citet{nissim2007smooth} is also related, which first randomly partitions a database into multiple small databases, performs the same algorithms on all the sub-databases, aggregates all the outputs, and finally adds randomness according to the smooth sensitivity of the aggregation function. For model-protection, the framework may be applicable for homogeneous tasks (which is the setting considered by DP-AGGR) to extend their method for empirical risk minimization: tasks instead of data instances can be randomly partitioned into groups to perform the above procedures. But it is not trivial to apply for heterogeneous tasks. The framework may also be applied to improve the utility of DP-AGGR by smoothed sensitivity.

}
   
   
\subsection{Methods Privately Releasing the Covariance Matrix}
Several methods have been proposed for the private release of the covariance matrix~\citep{jiang2016wishart,dwork2014analyze,blocki2012johnson}. Considering an additive noise matrix, according to our utility analysis, the overall utility of the MTL algorithm depends on the spectral norm of the noise matrix. A list of the bounds on the spectral norms of additive noise matrices can be found in~\citet{jiang2016wishart}. We choose to add Wishart noise~\citep{jiang2016wishart} to the covariance matrix for four reasons: (1) For a given privacy budget, this type of noise matrix has a better spectral-norm bound than that of Laplace noise matrix~\citep{jiang2016wishart}. (2) Unlike Gaussian noise matrix which enables an $(\epsilon,\delta)$-private method with a positive $\delta$, this approach enables an $(\epsilon,0)$-private method and can be used to build an iterative method that is entirely $(\epsilon,0)$-private, which provides a stronger privacy guarantee. (3) Unlike in the case of Gaussian and Laplace noise matrices, Wishart noise matrix is positive definite, which can be exploited to guaranteed that our method will not underperform comparing with STL methods under high noise level. (4) This approach allows arbitrary changes to any task, unlike the method of~\citet{blocki2012johnson}. %The usage of the perturbed covariance matrix depends on the specific MTL method applied.

==> discussion_conclusion.tex <==

\section{Conclusions}
\label{sec:conclusion}
In this paper, we discussed the potential security risks of multi-task learning approaches and presented a rigorous mathematical formulation of the model-protected multi-task learning (MP-MTL) problem. We proposed an algorithmic framework for implementing MP-MTL along with two concrete instantiations of this framework, which learn the low-rank and group-sparse patterns in the model matrix. {We demonstrated that our algorithms are guaranteed not to underperform comparing with single-task learning methods under high noise level. Privacy guarantees were also provided. Utility analyses suggested that both the strong-convexity condition and the acceleration strategy improve the utility bounds, {\color{blue} and that the acceleration strategy also improves run time}. A utility analysis for privacy-budget allocation yielded a recommendation for privacy budgets that are non-decreasing over the iterations. Experiments demonstrated that our algorithms significantly outperform baseline methods constructed by existing privacy-preserving MTL methods on the proposed model-protection problem.} Some interesting future directions of research include developing concrete MP-MTL algorithms for other MTL approaches and other optimization schemes.


==> experiments.tex <==
\section{Experiments}\label{sec:exp}

In this section, we evaluate the proposed MP-MTL method. As two instantiations of our method, Algorithm \ref{alg:MP-MTL-LR} and Algorithm \ref{alg:MP-MTL-GS} are evaluated with respect to their ability to capture the low-rank and group-sparse patterns, respectively, in the model matrix.
%The extensions to consider decomposed model-matrix are also discussed.
We use both synthetic and real-world datasets to evaluate these algorithms. All the algorithms were implemented in MATLAB.

\subsection{Methods for Comparison}
We use the least-square loss and the logistic loss for least-square regression and binary classification problems, respectively.

For each setting, we evaluate three types of methods: 1) non-private STL methods, in which each task is learned independently without the introduction of any perturbation; 2) {\color{blue}MP-MTL methods, including our proposed MP-MTL methods and baseline MP-MTL methods constructed by IP-MTL methods}; and 3) non-private MTL methods, corresponding to the original MTL methods without the introduction of any perturbation.

%Specifically, we use $\ell_2$ norm penalized method to be the non-private STL method for comparison with Algorithm \ref{alg:MP-MTL-LR} and use $\ell_1$ norm penalized method to be the non-private STL method for comparison with Algorithm \ref{alg:MP-MTL-GS}. For non-private MTL methods, we adopt the method of~\citet{ji2009accelerated} for comparison with Algorithm \ref{alg:MP-MTL-LR} and the method of~\citet{liu2009multi} for comparison with Algorithm \ref{alg:MP-MTL-GS}.


To select IP-MTL methods for constructing baseline MP-MTL methods, because few such approaches have been proposed, we firstly consider the DP-MTRL method proposed by~\citet{gupta2016differentially}. The authors of this method did not consider the increase in privacy loss resulting from their iterative update procedure. This problem is solved in our comparison by using the same composition technique as in our method.


%For comparison with existing differentially private MTL methods, because few such approaches have been proposed, we firstly consider the Differentially Private Multi-Task Relationship Learning (DP-MTRL) method proposed by~\citet{gupta2016differentially}. The authors of this method did not consider the increase in privacy loss resulting from their iterative update procedure. This problem is solved in our comparison by using the same composition technique as in our method (Equation \ref{eq:set_eps}).

We have also modified the DP-MTRL method to consider the Lipschitz constants of the loss functions when computing the sensitivities in the $4$-th step of the algorithm, which were omitted in the Algorithm 1 presented in the cited paper. For all $i\in[m]$, the Lipschitz constant $L_i$ of the loss function $\calL_i$ is estimated as $L_i = \max_{j\in[n_i]}|\calL'_i(\x_{ij}\w_i,y_{ij})|$, which is smaller than the true value. Thus, intuitively, we add less noise in their algorithm than should be added. %By contrast, our MP-MTL methods do not need to consider the Lipschitz constants of the loss functions.
%%%Editor - Please ensure that the intended meaning has been maintained
%%%in the above edit.

{In the case of binary classification, we let DP-MTRL still minimize the least-square loss}, because in each of its outer iterations (which alternately compute the parameter matrix and its covariance matrix), DP-MTRL requires a closed-form solution to guarantee the theoretical privacy results. However, for the logistic loss, iterative optimization is required in each outer iteration; consequently, the requirement of a closed-form solution cannot be satisfied. Therefore, DP-MTRL provides no privacy guarantee for the logistic loss. Moreover, it is not trivial to modify the DP-MTRL algorithm for loss functions that require iterative optimization in each outer iteration because additional leakage will occur in each inner iteration.

The DP-AGGR method proposed by~\citet{pathak2010multiparty} which outputs an averaged model as the final solution, is also considered as an IP-MTL method to transform into a baseline MP-MTL method.

\begin{remark}
{\color{blue}The baseline MP-MTL methods constructed by IP-MTL methods, DP-MTRL and DP-AGGR, are still referred to as their respective names.}
\end{remark}


%The differentially private aggregation (DP-AGGR) method proposed by~\citet{pathak2010multiparty}, which outputs an averaged model as the final solution, is also considered for comparison.
 
 

%Note that we only use DP-MTRL to compare with respect to the least square loss because in each outer iteration (to alternatively compute the parameter matrix and its covariance matrix), DP-MTRL requires a closed-form solution to guarantee the theoretical results for privacy. In contrast, for the logistic loss, one requires iterative optimization at each outer iteration so that such a requirement of a closed-form solution cannot be satisfied. As such, DP-MTRL provides no privacy guarantee for the logistic loss. Moreover, it is not trivial to modify their DP-MTRL for loss functions that need iterative optimization in each outer iteration because additional leakage will occur at each inner iteration. Therefore, we do not compare the method in such a setting.

%We also considered comparing the method proposed by~\citet{pathak2010multiparty}, which uses an averaged model to share information across tasks. However, because it only performs averaging, the ability to cover varying levels of the relatedness of tasks is limited. Moreover, the method even often underperforms STL methods in our experiment. As such, the results of this method are not reported.

Differentially private STL methods are not considered because 1) empirically, they are always outperformed by non-private STL methods~\citep{chaudhuri2011differentially, wang2015privacy}, and 2) our MP-MTL method always outperforms STL methods, as will be presented later.

\subsection{Experimental Setting}


For the non-private methods, the regularization parameters and the numbers of iterations were optimized via $5$-fold cross-validation on the training data{, and acceleration was used without considering the strong convexity of the loss function $f$}. {For the private methods, the regularization parameters, the number of iterations, the optimization strategy (whether to use acceleration and whether to consider strong convexity via adding $\ell_2$ norm penalties), and the privacy-budget allocation hyper-parameters ($\alpha$ and $Q$) under each privacy loss $\epsilon$ were optimized via $5$-fold cross-validation on the training data. In the case where strong convexity was considered, $\frac{\mu}{2}\|\w_i\|_2^2$ was added to each $\mathcal{L}_i$ with $\mu = 1e-3$.}

{\color{blue}Note that the parameter tuning step using cross-validation was not included in the privacy budget for the algorithms. In this paper, we regarded the hyper-parameters generated by cross-validation as given for not only our methods, but also the baseline methods (DP-AGGR and DP-MTRL). An effective cross-validation method using the minimum privacy budget with the optimum utility will be explored in our future work.}


For all the experiments, the $\delta$ values in the MP-MTL algorithms were set to {$1/m\log(m)$}, where $m$ is the number of tasks, as suggested by~\citet{abadi2016deep}, and the $\delta$ values in the baseline MP-MTL methods, i.e., DP-MTRL and DP-AGGR, were set in accordance with Proposition \ref{th:prop_DP-MP-iter}.
%%%Editor - Please consider whether DP-AGGR should also be included in the
%%%sentence above, as follows: ``the values of $\delta$ for the DP-MTL methods,
%%%i.e., DP-MTRL and DP-AGGR, were set...''

%We use a homogeneous privacy loss for the iterative algorithms, i.e., we set $\epsilon_1=\cdots=\epsilon_T$ for \eqref{eq:set_eps}.

%The averaging technique in Algorithm \ref{alg:MP-MTL-LR} and Algorithm \ref{alg:MP-MTL-GS} is not adopted, i.e., we set $t_0=T$ for both algorithms, since the utility is not ideal in our experiment.

%For the optimization, we adopt Nesterov’s accelerated method used in~\citet{ji2009accelerated} and~\citet{ji2009accelerated} with a fixed step size of $\eta$.

All experiments were replicated 100 times under each model setting.

\subsection{Evaluation Metrics}

{We adopt evaluation metrics commonly-encountered in MTL approaches.} For least-square regression, we use the nMSE~\citep{chen2011integrating,gong2012robust}, which is defined as the mean squared error (MSE) divided by the variance of the target vector as the evaluation criterion. For binary classification, we use the average AUC~\citep{chen2012learning}, which is defined as the mean value of the area under the ROC curve for each task.


\subsection{Simulation}

We created a synthetic dataset as follows. The number of tasks was {$m = 320$}, the number of training samples for each task was {$n_i = 30$},
and the feature dimensionality of the training samples was {$d = 30$}.
The entries of the training data $\X_i \in \mathbb{R}^{ n_i\times d}$ (for the $i$-th
task) were randomly generated from the normal distribution $\mathcal{N}(0, 1)$ before being normalized such that the $\ell_2$ norm of each sample was one.

{To obtain a low-rank pattern, a covariance matrix $\SSigma \in \mathbb{R}^{m\times m}$ was firstly generated, as shown in Fig. \ref{fig:syn_relation} (a). Then the model parameter matrix $\W\in\mathbb{R}^{d\times m}$ (see Fig. \ref{fig:syn_relation} (d)) was generated from a Matrix Variate Normal (MVN) distribution~\citep{gupta1999matrix}, i.e., $\W\sim MVN(\mathbf{0},\I,\SSigma)$.}

To obtain a group-sparse pattern, the model parameter matrix $\W\in\mathbb{R}^{d\times m}$ was generated such that the first $4$ rows were non-zero. The values of the non-zero entries were generated from a uniform distribution in the range $[-50, -1]\bigcup [1, 50]$. %We set $n_i = 30$ in this setting.

Without loss of generality, we consider only the simulation of least-square regression. The results for logistic regression are similar. The response (target) vector for each task was $\y_i = \X_i\w_i + \varepsilon_i \in \mathbb{R}^{n_i} (i \in [m])$, where each entry in the vector $\varepsilon_i$ was randomly generated from $\mathcal{N} (0, 1)$.

The test set was generated in the same manner; the number of test samples was $9n_i$.

\begin{figure}[t!]
\centering
\subfigure[True]{\includegraphics[width=1.1in]{relation_true}}
\subfigure[DP-MTRL]{\includegraphics[width=1.1in]{relation_after_add_noise_DPMTRL}}
\subfigure[MP-MTL]{\includegraphics[width=1.1in]{relation_after_add_noise}}
\subfigure[True]{\includegraphics[width=1.1in]{W_true}}
\subfigure[DP-MTRL]{\includegraphics[width=1.1in]{W_after_add_noise_DPMTRL}}
\subfigure[MP-MTL]{\includegraphics[width=1.1in]{W_after_add_noise}}
\caption{Task relationships and output model matrices for the synthetic data experiments: (a), (b) and (c) are task relationship matrices, (d), (e) and (f) are the output model matrices. The results shown are the average of $100$ runs with $\epsilon = 0.1$.}\label{fig:syn_relation}
\end{figure}


%Non-private STL methods provide the worst nMSE scores because they do not take advantage of knowledge across tasks. On the other hand, non-private MTL methods provide the best scores because no noise is introduced in the learning process.

{
\subsubsection{Privacy Budget Allocation}\label{sec:exp_ba_simu}
The privacy-budget allocation strategies in Section \ref{subsec:Budget} were evaluated based on the synthetic data associated with the low-rank model matrix. The results shown in Fig. \ref{fig:syn_budget_allocation} are from $5$-fold cross-validation on the training data. The prediction performances increase when acceleration is used, and achieve local optima at small positive values of the horizontal axes, which is consistent with our utility analyses. A local optima exists in the negative horizontal axis in Fig. \ref{fig:syn_budget_allocation} (b) when acceleration is used---perhaps because $m$ is not large enough as assumed in Assumption \ref{th:asm_m}.
\begin{figure}[t!]
\centering
\subfigure[Convexity]{\includegraphics[width=1.7in]{BA_convex}}
\subfigure[Strong convexity]{\includegraphics[width=1.7in]{BA_strong_convex}}
\caption{Evaluations for privacy-budget allocation strategies. In (a), we set $\epsilon_t = \Theta(t^{\alpha})$, for $t\in[T]$; in (b), we set $\epsilon_t = \Theta(Q^{-t})$, for $t\in[T]$. $Q_0 = 1-\sqrt{\mu} \approx 0.9684$. The results shown are averages of $100$ runs with $\epsilon = 0.1$. For the non-private MTL method, the nMSE was $0.0140$.  }\label{fig:syn_budget_allocation}
\end{figure}
}
{
\subsubsection{Noise-To-Signal Ratio}
Based on the setting in Section \ref{sec:exp_ba_simu},  noise-to-signal ratios under the best privacy-budget allocation strategy (using acceleration and considering basic convexity) are shown in Fig. \ref{fig:syn_noise_ratio}, {\color{blue}in which we run Algorithm 2 on the synthetic data set with the low-rank pattern.}  In contrast, for DP-MTRL, $\log_{10}(\|\E\|_F/\|\widetilde{\SSigma}^{(t)}\|_F) = 0.2670\pm 0.0075$ with the best iteration number $T=1$. The output model matrices of both DP-MTRL and our method are shown in Fig. \ref{fig:syn_relation} (e) and (f), respectively, along with their respective covariance matrices shown in Fig. \ref{fig:syn_relation} (b) and (c). These plots suggest that high level of noises added in our method had little influence on the output model matrix and the pattern in its covariance matrix, because our method adds noise only to the knowledge-sharing process and our method degrades to an STL method under high noise level (as shown in Proposition \ref{th:prop_better_than_STL}). {\color{blue}In contrast, in DP-MTRL, the output model matrix and the pattern in the covariance matrix were significantly affected and even destroyed because the noise was added directly to the model matrix, which resulted in negative side-effects. It may also because DP-MTRL is \emph{a local private learning algorithm}, which need much larger $m$ to achieve acceptable utility; see the discussion in Section \ref{subsec:related_def}.}
\begin{figure}[t!]
\centering
\subfigure{\includegraphics[width=1.7in]{noise_ratio}}
\caption{Noise-to-signal ratio over the iterations of Algorithm \ref{alg:MP-MTL-LR}. The results shown are averages of $100$ runs with $\epsilon = 0.1$.}\label{fig:syn_noise_ratio}
\end{figure}
}

{
\subsubsection{Privacy-Accuracy Tradeoff}
In Fig. \ref{fig:syn}, the performances of both of our MP-MTL algorithms (i.e., Algorithms \ref{alg:MP-MTL-LR} and \ref{alg:MP-MTL-GS}) fall between those of the non-private STL and non-private MTL methods, suggesting that our methods are useful as MTL methods but may be affected by the introduced noise. In Fig. \ref{fig:syn} (a), Algorithm \ref{alg:MP-MTL-GS} underperforms comparing with Algorithm \ref{alg:MP-MTL-LR}, because the true model matrix is not group-sparse. DP-MTRL outperforms the STL method and our Algorithm \ref{alg:MP-MTL-GS} when $\epsilon$ is large, because it suits the true model matrix, in which the relatedness among tasks is modeled by a graph. In Fig. \ref{fig:syn} (b), the true model matrix is group-sparse and is not suitable for DP-MTRL, hence DP-MTRL underperforms comparing with the STL method even when $\epsilon$ is large. Algorithm \ref{alg:MP-MTL-LR} rivals Algorithm \ref{alg:MP-MTL-GS}, because the true model matrix is also low-rank. In both panels of Fig. \ref{fig:syn}, Algorithm \ref{alg:MP-MTL-LR} rivals the non-private MTL when $\epsilon = 10$.

\begin{figure}[t!]
\centering
\subfigure[Low-rank pattern]{\includegraphics[width=2.7in]{simu_relation_2}}
\subfigure[Group-sparse pattern]{\includegraphics[width=2.7in]{simu_groupsparse_2}}
\caption{Privacy-accuracy tradeoff on synthetic datasets. For (a), the data associated with the low-rank model matrix were used; for (b), the data associated with the group-sparse model matrix were used. MP-MTL-LR denotes Algorithm \ref{alg:MP-MTL-LR}, MP-MTL-GS denotes Algorithm \ref{alg:MP-MTL-GS}, and STL denotes the $\ell_2$-norm-penalized STL method. In both panels, STL and MTL denote non-private methods. In (b), the nMSEs of DP-MTRL are above $0.16$; in both panels, the nMSEs of DP-AGGR are above $0.78$. More detailed performances of DP-MTRL and DP-AGGR are presented in Fig. \ref{fig:syn_detail_baseline}.}\label{fig:syn}
\end{figure}
}

{\color{blue}
 
In Fig. \ref{fig:syn_detail_baseline}, the detailed performances of DP-MTRL and DP-AGGR are shown, which correspond to those in Fig. \ref{fig:syn}. Fig. \ref{fig:syn_detail_baseline} (c) is used to show that the accuracy of DP-AGGR grows with $\epsilon$ under the same setting as in Fig. \ref{fig:syn_detail_baseline} (b). As we discussed, DP-AGGR only performs model-averaging, which is not suitable for the true model matrices in both settings of Fig. \ref{fig:syn_detail_baseline} (a) and (b), hence the accuracies of DP-AGGR are much worse than those of the respective STL methods.

\begin{figure}[t!]
%\centering
\subfigure[Low-rank pattern]{\includegraphics[width=1.7in]{simu_relation_2_DPMTRL_DPAGGR}}
\subfigure[Group-sparse pattern]{\includegraphics[width=1.7in]{simu_groupsparse_2_DPMTRL_DPAGGR}}
\subfigure[Group-sparse pattern]{\includegraphics[width=1.7in]{simu_groupsparse_2_DPAGGR_only}}
\caption{Detailed privacy-accuracy tradeoff on synthetic datasets for DP-MTRL and DP-AGGR. For (a), the data that associated with the low-rank model matrix were used; for (b) and (c), the data that associated with the group-sparse model matrix were used. In (c), the plot shows the same performances of DP-AGGR as in (b) with a finer vertical axis. Other settings are the same as in Fig. \ref{fig:syn}.}\label{fig:syn_detail_baseline}
\end{figure}
}


{
\subsubsection{Varing the Number of Tasks}
Based on the setting in Section \ref{sec:exp_ba_simu}, the average performances of the first $20$ tasks out of the $320$ tasks are shown in Fig. \ref{fig:syn_multim} under different numbers of tasks for training. The accuracy increases with the number of involved tasks, which is consistent with our utility analyses. {\color{blue}Note that the standard deviation of each result is plotted in Fig. \ref{fig:syn_multim}. Therefore, the increments are statistically significant.} 


\begin{figure}[t!]
\centering
\subfigure{\includegraphics[width=2.7in]{multim}}
\caption{Behaviors based on the number of tasks $m$ used for training. MTL used $320$ tasks for training.}\label{fig:syn_multim}
\end{figure}
}



\subsection{Application}


\subsubsection{Data Description}

We also evaluate the considered methods on the following two real datasets.

\noindent\textbf{\emph{\underline{School Data}}}. The School dataset\footnote{http://www.cs.ucl.ac.uk/staff/a.argyriou/code/} is a popular dataset for MTL~\citep{gong2012robust} that consists of the exam scores of 15,362 students
from 139 secondary schools. Each student is described by 27 attributes, including both school-specific and student-specific information, such as gender and ethnic group.
The problem of predicting exam scores for the students can be formulated as an MTL problem: the number of tasks is $m=139$, the data dimensionality is $d=27$, and the number of data samples is $\sum_in_i = 15,362$.
%In our experiments, we randomly selected 30\% of the samples (from each task) to form the training set and used the remaining samples as the test set.

\noindent\textbf{\emph{\underline{LSOA II Data}}}. These data are from the Second Longitudinal Study of Aging (LSOA II) \footnote{https://www.cdc.gov/nchs/lsoa/lsoa2.htm.}. LSOA II was a collaborative study conducted by the National Center for Health Statistics (NCHS) and the National Institute of Aging from 1994 to 2000. A national representative sample of $9,447$ subjects of $70$ years of age and older were selected and interviewed. Three separate interviews were conducted with each subject, one each during the periods of 1994-1996, 1997-1998, and 1999-2000, and referred to as WAVE 1, WAVE 2, and WAVE 3, respectively. Each wave of interviews included multiple modules covering a wide range of assessments. We used data from WAVE 2 and WAVE 3, which include a total of $4,299$ sample subjects and 44 targets (each subject corresponded to 44 targets), and $188$ features were extracted from the WAVE 2 interviews.
{
The targets include $m=41$ binary outcomes used in this study. These outcomes fall into several categories: 7 measures of fundamental daily activity, 13 of extended daily activity, 5 of social involvement, 8 of medical condition, 4 of cognitive ability, and 4 of sensation condition.

The features include records of demographics, family structure, daily personal care, medical history, social activity, health opinions, behavior, nutrition, health insurance and income and assets, the majority of which are binary measures.

Both the targets and the features have missing values due to non-response and questionnaire filtering. The average missing value rates of the targets and features are 13.7\% and 20.2\%, respectively. To address the missing values among the features, we adopted the following preprocessing procedure. For the continuous features, missing values were imputed with the sample mean. For binary features, it is better to treat the missing values as a third category, as the absence of a value may also carry important information. Therefore, two dummy variables were created for each binary feature with missing values (no third variable is necessary in such a case). This resulted in a total of $d=295$ features. To address the missing values among the targets, we include the samples associated with observed targets for each task, resulting in $\max_{i\in[m]}n_i = 3,473$.

%Ultimately, data from $n = 3988$ individuals were included in this study. The MTL problem can be formulated as follows: the number of binary classification tasks is $m=41$, the data dimensionality is $d=295$, and the sample sizes are $n_1=\ldots=n_{41} = n$. Each feature vector (belonging to one individual) is shared among all tasks.
}

%These data are from the Second Longitudinal Study of Aging (LSOA II) \footnote{Source: National Center for Health Statistics (2002)}~\citep{LSOA2002}. LSOA II was a collaborative study by the National Center for Health Statistics (NCHS) and the National Institute of Aging conducted from 1994-2000. The national representative sample consisted of $9447$ individuals $70$ years of age and older, who were selected and interviewed. Three separate interviews were conducted during the periods of 1994-1996, 1997-1998, and 1999-2000,. The interviews are referred to as WAVE 1, WAVE 2, and WAVE 3 interviews, respectively. Each wave of interviews included multiple modules covering a wide range of assessments. In this paper, we used data generated from the WAVE 2 and WAVE 3 interviews.

%A total of $4299$ individuals attended the WAVE 2 and WAVE 3 interviews.
%The interviews provided several filtering and quality control questions, including ``respondent deceased during the interview period'', ``respondent intellectually capable of conducting interviews'', ``respondent could understood questions'', and ``respondent gave answers reasonably accurate''. We used these questions to filter out deceased and low-quality sample individuals.

%We built predictive models using the WAVE 2 data as the predictors and the sample individuals' conditions in WAVE 3 as the targets.
%Based on a literature review on comprehensive geriatric risk assessment and available interview questions, $41$ {binary} targets were extracted from the WAVE 3 data.

%A multi-task learning problem can therefore be formulated as: task number $m=41$, data dimension $d=27$, and data sample size $\sum_in_i = 15362$

For both the real-world datasets, We randomly selected 30\% of the samples (from each task) to form the training set and used the remaining samples as the test set. For all tasks, each data point was normalized to have unit length.



\subsubsection{Privacy-Accuracy Tradeoff}
From Fig. \ref{fig:real}, we can observe results similar to those seen in Fig. \ref{fig:syn}. In addition, our MP-MTL algorithms outperform the baseline MP-MTL methods, DP-MTRL and DP-AGGR, especially when $\epsilon$ is small. 
%This is because DP-MTRL and DP-AGGR introduce excessive noise to protect the model and all data instances of every individual task simultaneously.
%%%Editor - Please consider whether ``every individual task'' would convey the
%%%intended meaning better than ``any single task''.
{DP-AGGR underperforms comparing with the STL method because its model averaging approach assumes that the tasks are homogeneous. In Fig. \ref{fig:real} (b), the aAUC values of DP-MTRL and our Algorithms (\ref{alg:MP-MTL-LR} and \ref{alg:MP-MTL-GS}) increase slowly because the feature dimension is large and the number of tasks is insufficient, which is consistent with our utility analyses.}
%%%Editor - Please note that results for DP-AGGR do not appear to be plotted
%%%in Fig. 4.

%Furthermore, MP-MTL-LR outperforms MP-MTL-GS on both datasets, which may suggest that feature selection via group-sparse regularization is easier to jeopardize than is feature transformation by low-rank regularization.

\begin{figure}[t!]
\centering
\subfigure[School Data]{\includegraphics[width=1.7in]{school_2}}
\subfigure[LSOA II Data]{\includegraphics[width=1.7in]{LSOA_2}}
\caption{Privacy-accuracy tradeoff on real-world datasets. In both panels, MTL denotes the method with the best performance among the four non-private MTL methods proposed by~\citet{ji2009accelerated},~\citet{liu2009multi},~\citet{zhang2010convex} and DP-AGGR without perturbations; MP-MTL-LR denotes Algorithm \ref{alg:MP-MTL-LR}, whereas MP-MTL-GS denotes Algorithm \ref{alg:MP-MTL-GS}; STL denotes the method with the better performance between the $\ell_1$- and $\ell_2$-regularized methods. In (b), aAUCs of DP-AGGR are below $0.66$. Detailed performances of DP-AGGR are presented in Fig. \ref{fig:real_detail_baseline}.}\label{fig:real}
\end{figure}



{\color{blue}
 
In Fig. \ref{fig:real_detail_baseline}, the detailed performances of DP-AGGR are shown. In Fig. \ref{fig:real_detail_baseline} (b), because the dimension is large and the number of tasks is not sufficient, the accuracy of DP-AGGR barely grows with $\epsilon$.

\begin{figure}[t!]
\centering
\subfigure[School Data]{\includegraphics[width=1.7in]{school_2_DPMTRL_DPAGGR}}
\subfigure[LSOA II Data]{\includegraphics[width=1.7in]{LSOA_2_DPMTRL_DPAGGR}}
\caption{Detailed privacy-accuracy tradeoff on real-world datasets for DP-AGGR. All the settings are the same as in Fig. \ref{fig:real}. }\label{fig:real_detail_baseline}
\end{figure}
}

{
Since the MTL behavior may change when the training-data percentage (the size of the training data divided by the size of the entire dataset) changes, we evaluated the methods on both real-world datasets at different training-data percentages and achieved similar results; see the supplementary material for more details.}


%{
%\subsubsection{Accuracy vs. Training-Data Percentage Tradeoffs}
%
%Since MTL behavior changes significantly when training-data percentage (the size of training data divided by the size of the whole dataset) changes, we evaluate the methods on both real-world datasets at different training-data percentage. We use a unified normalized score below to evaluate all the methods based upon the performances of the non-private STL method and non-private MTL method in each setting.
%\begin{align}\label{eq:norm_score_percent}
% s_{\mbox{norm}} = \frac{s_{\mbox{priv}}-s_{\mbox{STL}}}{s_{\mbox{MTL}}-s_{\mbox{STL}}},
%\end{align}
%where $s_{\mbox{STL}}$ denotes the average performance of the non-private STL method, $s_{\mbox{MTL}}$ denotes the average performance of the non-private MTL method and $s_{\mbox{priv}}$ denotes the average performance of the private method for evaluation, which can be any of our MP-MTL methods or the DP-MTRL method. The performance used can be average AUC or nMSE. The larger the normalized score implies the better performance of the evaluated method. Such normalized score described the relative prediction performance of the evaluated method.
%
%Here we only use our low-rank method MP-MTL-LR, because it always outperforms our group-sparse method MP-MTL-GS in the above experiments.
%
%From Fig. \ref{fig:real_percent}, we can observe that, our MP-MTL method behaves similarly at different training-data percentage on the School dataset, while on the Patient Survey dataset, performances are best when training-data percentage equals 30\% and are worst when training-data percentage equals 90\%, which is because 1) the relative advantage of MTL over STL is significant when the training-data percentage is small; 2) the average data-size of the Patient Survey dataset is much bigger than that of the School dataset, thus advantage of MTL over STL is more likely to be saturated when the training-data percentage is large. At each training-data percentage, our MP-MTL method outperforms DP-MTRL, especially when $\epsilon$ is small.
%
%
%\begin{figure}[t!]
%\centering
%\subfigure[School Data]{\includegraphics[width=2.3in]{school_percent}}
%\subfigure[Patient Survey Data]{\includegraphics[width=2.3in]{LSOA_percent}}
%\caption{{Algorithm performance on real-world datasets at different training-data percentage. The normalized score is defined in \eqref{eq:norm_score_percent}. MTL denotes the performance of the non-private MTL methods proposed by~\citet{ji2009accelerated}. MP denotes our low-rank method MP-MTL-LR, and DP denotes DP-MTRL. $r$ denotes the training-data percentage.}}\label{fig:real_percent}
%\end{figure}
%
%}









==> model.tex <==
\section{Methodology}\label{sec:method}

%We present our methodologies in this section: the modeling and {rationale} of our model-protected multi-task learning (MP-MTL) framework, the technique used to realize our MP-MTL framework, two instantiations of MP-MTL used to learn the low-rank pattern and group-sparse pattern of the model matrix, and the relationships between our work and other differentially private multi-task learning approaches.

We present our methodology in this section: the modeling of and {rationale} for our MP-MTL framework, two instantiations and utility analyses. Regarding the theoretical results, we present only the main results; the detailed derivations are deferred to the provided supplementary material.
%one extended framework when decomposed model matrix is considered.


%\subsection{Preliminaries}
%First we summarize the notations and symbols that will be used throughout the paper in Table \ref{tab:notations}, and then introduce the basic concepts in differential privacy according to \cite{chaudhuri2011differentially} along with the formulations of multi-task learning that we will be focusing on.\\[-.5em]

%\begin{table}
%\centering
%\caption{Notations and Symbols}
%\label{tab:notations}
%{\small
%\begin{tabular}{l|p{20em}}
%\hline\hline $[k]$& the index set $\{1,2,\cdots,k\}$\\
%\hline
%$[-i]$& the index set by taking out index $i$\\
%\hline $\|\cdot\|_{*}$& the trace norm of a matrix (sum of the matrix's singular values)\\
%%\hline $\|\cdot\|_F$& the Frobenius norm of a matrix (sum of the square of all elements in the matrix)\\
%%\hline $\|\cdot\|_{1}$& $\ell_1$-norm of a matrix (sum of the absolute value of all elements in the matrix)\\
%\hline\hline
%\end{tabular}}
%\end{table}

%\subsection{Differential privacy}
%The following defenition is according to \cite{chaudhuri2011differentially} .
%\begin{definition}
%\noindent{\bf Definition 1} {\em An algorithm $\mathcal{A}$ provides $(\epsilon, \delta) $ - differential privacy if for any two data sets $\mathcal{D}$ and $\mathcal{D}'$ which differ in a single entry and for any set $\mathcal{S}$ :
% \begin{align*}
% \mathbb{P}(\mathcal{A}(\mathcal{D})\in \mathcal{S})
% \leq  \exp(\epsilon)\mathbb{P}(\mathcal{A}(\mathcal{D}')\in \mathcal{S}) + \delta
% \end{align*}
% where $\mathcal{A}(\mathcal{D})$ or $\mathcal{A}(\mathcal{D}')$) is the output of $\mathcal{A}$ on input $\mathcal{D}$ or $ \mathcal{D}' $.}
%\end{definition}


%In our case, if we consider the output of $\mathcal{A}$ as the model parameters $\mbox{\boldmath$\theta$}$ we want to learn, then we can use the another form of definition using its posterior as follows \cite{wang2015privacy}.\\[-.5em]
%Let $\mathcal{A}$ be some differentially private learning algorithm, and $\mbox{\boldmath$\theta$}$ be the model parameters that we want to learn, then we can use the following definition to measure how much privacy can $\mathcal{A}$ preserve \cite{wang2015privacy}.\\[-.5em]
%
%\noindent{\bf Definition 1}. {\em  An algorithm $\mathcal{A}$ provides $(\epsilon,\delta)$ - differential privacy if for any two data sets $\mathcal{D}$ and $\mathcal{D}'$, which are inputs of $\mathcal{A}$, differ in a single data point, any parameter $\ttheta$ which is a solution of $\mathcal{A}$, and some constants $\epsilon,\delta\geq 0$, we have
% \begin{align*}
%p(\ttheta | \mathcal{D}  )
% \leq  \exp(\epsilon)p(\ttheta | \mathcal{D}' ) + \delta.
% \end{align*}}%\vspace{-1em}
%Note that the defined algorithm $\mathcal{A}$ is randomized; the output parameter $\ttheta$ is a random variable whose distribution is conditioned on the data set $\mathcal{D}$ or $\mathcal{D}'$. And the privacy loss pair $(\epsilon,\delta)$ quantifies the privacy-risk of the algorithm $\mathcal{A}$. We can set $\epsilon$ and $\delta$ to be smaller to force the two posterior distributions $p(\ttheta | \mathcal{D}  )$ and $p(\ttheta | \mathcal{D}' ) $ to be more similar, which makes it harder for an attacker to know whether some certain data point is changed (or enters into the data set $\mathcal{D}$) based on the variation of the posterior distribution. Therefore, although the participation of a new data point of some user will bring new information into the output parameter $\ttheta$, it is hard for an attacker to know the information of the new data point of the user by comparing the difference between the old and new output distributions of parameter $\ttheta$. Thus we can lower the privacy-risk by smaller $\epsilon$ and $\delta$.

%And for multi-task learning, the basic formulation that we will work on is as follows.
%\begin{equation}\label{eq:MTL_ONE}
%\min_{\W} \sum\nolimits_{i=1}^m\calL_i(\X_i\w_i,\y_i) + \lambda_g g(\W),
%\end{equation}
%where $m$ is the number of tasks. Data sets of the tasks are denoted by $(\X^m,\y^m) = \{(\X_1,\y_1),\ldots,(\X_m,\y_m)\}$, where for each $i\in[m]$, $\X_i\in \mathbb{R}^{n_i \times d}$ and $\y_i\in \mathbb{R}^{n_i \times 1} $ denote the data matrix and target vector of the $i$-th task with $n_i$ samples and dimensionality $D$, respectively, and $\calL_i$ is the prediction loss function of the $i$-th task. In this paper, we will focus on linear MTL models and $\w_i$ is the decision vector for task $i$ and
%$\W=[\w_1,\w_2,\cdots,\w_m]\in \mathbb{R}^{d \times m}$ denotes the model parameter matrix. To explicitly separate out the shared components and individual components of $\W$, a popular strategy is to decompose $\W=\P+\Q$, where some useful information shared across $m$ tasks is contained in $\P=[\p_1,\p_2,\cdots,\p_m]$. And $\Q=[\q_1,\q_2,\cdots,\q_m]$ is the individual effect concatenated over $m$ tasks. Then we can obtain the model parameters by solving the following optimization problem.
%\begin{eqnarray}\label{eq:MTL_TWO}
%&\min_{\W}& \sum\nolimits_{i=1}^m\calL_i(\X_i\w_i,\y_i) + \lambda_g g(\P) + \lambda_h \sum\nolimits_{i=1}^m h(\q_i)\nonumber \\
%&s.t.& \W = \P+ \Q
%\end{eqnarray}
%In Problem (\ref{eq:MTL_ONE}) and Problem (\ref{eq:MTL_TWO}), $g(\cdot)$ denotes some norm that represents the structure of shared information among tasks, where one popular choice is the trace norm $\|\cdot\|_{*}$ \cite{ando2005framework}\cite{ji2009accelerated}\cite{chen2011integrating}. $h(\cdot)$ denotes some regularizer imposed on individual task effects, such as $\ell_1$-norm \cite{jalali2010dirty} and $\ell_2$-norm \cite{ando2005framework}\cite{gong2012robust}.

%In Problem (\ref{eq:MTL_ONE}), it is always assumed that some structure captured by $g(\cdot)$ are shared among all tasks. While in Problem (\ref{eq:MTL_TWO}), multi-task learning algorithm simultaneously share information among tasks and minimize another norm to learn the information specific to each task.


%\subsection{Differentially private multi-task learning}

\subsection{The General Framework for MP-MTL}
%We first present our main ideas for modeling our MP-MTL framework in the non-iterative setting before extending it to the general iterative setting.
 
Consider an MTL algorithm $\calA$ with a number of iterations $T$. For $t = 1,\ldots,T$, a trusted curator collects the models of $m$ tasks, respectively, denoted by $\w_1^{(t-1)},\ldots,\w_m^{(t-1)}$. Then, a model-protection and shared-information-extraction procedure is performed, and the updated models $\hat{\w}_1^{(t)},\ldots,\hat{\w}_m^{(t)}$ are output and sent back to their respective tasks.
 
\begin{remark}\label{th:rm_nodata}
{\color{blue}Note that in each iteration, the curator collects the models only. The dataset of each task can be regarded as input for the entire MTL algorithm, but is not the input for the curator.}
\end{remark}

In such a setting, for each $i\in[m]$, we wish to protect the dataset $\calD_i = (\X_i,\y_i)$ of task $i$ and its \emph{entire input model-sequence} $(\w_{i}^{(0)},...,\w_{i}^{(T-1)})$ (denoted by $\w_{i}^{(0:T-1)}$ for short). {\color{blue}\emph{For the $i$-th task}, the \emph{entire output model-sequence} of other tasks, $\hat{\w}_{[-i]}^{(1:T)}$, is the \emph{view} of a potential adversary, i.e., the information that s/he can acquire to infer the unique information of task $i$. Note that although the output model-sequence of each task is what we ultimately wish to protect, the unique information within which of the task is contained in the task's dataset and input model-sequence, which are actually protected.}
 

%As such, for the $i$-th task ($i\in[m]$), we assume that potential adversaries may acquire $\hat{\w}_{[-i]}$, and  \emph{we wish to protect} both the \emph{input model} $\w_{i}$ and the dataset $\calD_i$. {Note that although we ultimately wish to protect $\hat{\w}_i$, i.e., the output model for the $i$-th task, all information related to the $i$-th task in $\hat{\w}_i$ comes from the input model $\w_{i}$ and the dataset $\calD_i$, and the latter are the only objects that any algorithm can directly control because they are the inputs.}

%For the sake of intuition, considering $T=1$, we set $\w'_i^{(0)}$ and $\calD'_i$ in Definition \ref{th:df_MP-MTL-simple} to $\mathbf{0}$ and the empty set, respectively; then, the goal of MP-MTL is to ensure that when the model for a new task is provided to the curator, an adversary, including other existing tasks, cannot discover significant anomalous information from the distribution of its \emph{view}: $\hat{\w}_{[-i]}^{(1)}$. Thus, the information on the new task's model is protected. Note that for different tasks, the views of an adversary are different. %Editor: Please ensure that the intended meaning has been maintained in this edit.



%We can redefine the MP-MTL algorithm in the form of differential privacy.
The idea to use tools of differental privacy is as follows.
{\color{blue}For simpilicity, consider $T=1$ and omit the iteration-step indices.} Let $\widetilde{\calD}  = \{(\w_1, \calD_1),\ldots,(\w_m, \calD_m)\}$ be an augmented dataset; i.e., let $(\w_i, \calD_i)$ be treated as the $i$-th ``data instance'' of the augmented dataset $\widetilde{\calD}$, for all $i\in[m]$. Thus, the $m$ datasets and $m$ models associated with the $m$ tasks are transformed into a single dataset $\widetilde{\calD}$ with $m$ ``data instances''. Then, we define $m$ outputs $\ttheta = (\theta_1,\ldots,\theta_m)$ such that for each $i\in[m]$, $\theta_i\in\calC_i$ denotes the \emph{view} of an adversary for task $i$, which includes $\hat{\w}_{[-i]}$. Then, an $(\epsilon,\delta)$ - MP-MTL algorithm $\calA(\calB)$ should satisfy $m$ inequalities:
%%%Editor - Please ensure that the intended meaning has been maintained
%%%in the above edit.
for each $i\in [m]$, for all neighboring datasets $\widetilde{\calD}$ and $\widetilde{\calD}'$ that differ by the $i$-th ``data instance'', and for any set $\calS_i\subseteq C_i$, we have
\begin{equation}\label{eq:MP_MTL-simple-dp}
\begin{split}
\bbP&( \theta_i \in \calS_i  \mid \calB = \widetilde{\calD}) \leq   e^{\epsilon} \bbP(\theta_i \in \calS_i  \mid \calB=\widetilde{\calD}') + \delta.
\end{split}
\end{equation}

We formally define an MP-MTL algorithm as follows.
\begin{definition}[MP-MTL]\label{th:df_MP-MTL-iter}
Let $\calA$ be a randomized MTL algorithm with a number of iterations $T$. In the first iteration, $\calA$ performs the mapping $(\W^{(0)} \in\mathbb{R}^{d\times m},\calD^m)\rightarrow \theta_1\in \calC_1$, where $\theta_1$ includes $\widehat{\W}^{(1)} \in\mathbb{R}^{d\times m}$. For $t=2,\ldots,T$, in the $t$-th iteration, $\calA$ performs the mapping $(\W^{(t-1)} \in\mathbb{R}^{d\times m},\calD^m,\theta_1,\ldots,\theta_{t-1})\rightarrow \theta_t\in \calC_t$, where $\theta_t$ includes $\widehat{\W}^{(t)} \in\mathbb{R}^{d\times m}$. $\calA$ is an \emph{$(\epsilon,\delta)$ - MP-MTL algorithm} if for all $i\in[m]$, for all $t\in[T]$, and for neighboring input pairs $(\W^{(t-1)},\calD^m)$ and $((\W')^{(t-1)},(\calD')^m)$ that differ only by the $i$-th task, such that $\w_i^{(t-1)}\neq (\w'_i)^{(t-1)}$ or $\calD_i\neq\calD'_i$, the following holds for some constants $\epsilon,\delta\geq 0$ and for any set $\calS \subseteq \mathbb{R}^{d\times (m-1)\times T}$:
\begin{equation}\label{eq:MP_MTL-iter}
\begin{split}
\bbP( &  \hat{\w}_{[-i]}^{(1:T)}  \in \calS  \mid \bigcap_{t=1}^T \calB_t = (\W^{(t-1)}, \calD^m, \ttheta_{1:t-1}) ) \\
\leq   &e^{\epsilon} \bbP(  \hat{\w}_{[-i]}^{(1:T)} \in \calS \mid \bigcap_{t=1}^T \calB_t = ((\W')^{(t-1)}, (\calD')^m, \ttheta_{1:t-1})) \\
&+ \delta,
\end{split}
\end{equation}
where for all $t\in[T]$, $\calB_t$ denotes the input for the $t$-th iteration and
\begin{numcases}{\ttheta_{1:t-1} = }
\nonumber \emptyset, & $t=1$\\
\nonumber \theta_1,\theta_2,\cdots,\theta_{t-1}, & $t\geq2$.
\end{numcases}
%and $\ttheta'$ is associated with the setting that the $i$th task has been replaced.
\end{definition}

{\color{blue}

Note that in Definition \ref{th:df_MP-MTL-iter}, we view the sequence of models, $\hat{\w}_{[-i]}^{(1:T)}$, as a single output of the algorithm for each task $i\in[m]$. The definition of neighboring inputs allows the model and dataset for any task to change on \emph{all rounds} of the iterative optimization, NOT only on a single round.
 
Definition \ref{th:df_MP-MTL-iter} defines a privacy constraint for MTL algorithms. Roughly speaking, this privacy constraint can be regarded identical to \emph{joint differential privacy} \citep{kearns2015robust,kearns2014mechanism} or \emph{one-analyst-to-many-analyst privacy} \citep{hsu2013differential}, despite differences of concepts between MTL, game theory, and database query.}

STL can be easily shown to be optimal for avoiding information leakage across tasks because the individual task models are learned independently.\vspace{-0.5em}
%\noindent{\bf Lemma 6}. {\em Any single task learning algorithm is a $(0,0)$ - MP-MTL algorithm.}\vspace{-1em}
{\color{blue}
\begin{claim}\label{th:lem_STL}
Any STL algorithm learns each task independently is a $(0,0)$ - MP-MTL algorithm.
\end{claim}\vspace{-0.5em}}
We learn from this claim that if there is no information sharing across tasks, then no leakage across tasks occurs.

 
Our MP-MTL framework is elaborated in Algorithm \ref{alg:MP-MTL}, where heterogeneous privacy budgets for different iteration steps are considered. {\color{blue}In order to render the total privacy budget less than a specified value using the adaptive composition theorem provided by~\citet{kairouz2017composition}, we define a composition bound of a series of privacy budgets as follows, in which the equation is directly taken from Theorem 3.5 of~\citet{kairouz2017composition}.

\begin{definition}[Composition Bound of Privacy Budgets]\label{th:df_com_bound}
For an integer $T\geq1$, a series of privacy budgets, $\epsilon_1,\ldots,\epsilon_T\geq0$, a specified privacy loss $\delta\geq 0$, the composition bound of $\{\epsilon_t\}$ is defined as $CB(\{\epsilon_t\},\delta)$, which equals
\begin{equation}\label{eq:set_eps}
\begin{split}
&\min\biggl\{ \sum_{t=1}^{T}\epsilon_t,\sum_{t=1}^{T}\frac{(e^{\epsilon_t}-1)\epsilon_t}{(e^{\epsilon_t}+1)}
+\sqrt{\sum_{t=1}^{T}2\epsilon_t^2\log\biggl(\frac{1}{\delta}\biggr)},\\
 &\sum_{t=1}^{T}\frac{(e^{\epsilon_t}-1)\epsilon_t}{(e^{\epsilon_t}+1)}
+\sqrt{\sum_{t=1}^{T}2\epsilon_t^2\log\biggl(e+\frac{\sqrt{\sum_{t=1}^{T}\epsilon_t^2}}{\delta}\biggr)}
\biggr\}.
\end{split}
\end{equation}
\end{definition}

}

In Algorithm \ref{alg:MP-MTL}, as mentioned in Section \ref{sec:pre}, we choose to protect the tasks' covariance matrix, which is denoted by $\SSigma= \W\W\trans$ or $\SSigma = \W\trans\W$, depending on the chosen MTL method. As previously stated, Wishart noise~\citep{jiang2016wishart} is added. Fig. \ref{fig:framework} illustrates the key concepts of the framework. {\color{blue}In detail, Step 1 of Algorithm \ref{alg:MP-MTL} ensures that the total privacy budgets satisfy the specified values $\epsilon$ and $\delta$, respectively. The purpose of norm clipping in Step 3 is just to render the models in a bounded space, which help us compute a proper scale of noise to add to satisfy the privacy constraint defined in Definition \ref{th:df_MP-MTL-iter}. Step 4 extracts shared information between tasks---the tasks' covariance matrix. Step 5 adds a perturbation into the shared information. Step 6 further extracts useful information in the perturbed covariance matrix. Step 7 sends the extracted useful information to each task to perform decoupled learning. If no noise is added, Steps 4-7 could be a proximal gradient descent step, i.e., first performing a proximal operator step and then taking a gradient descent step; see, e.g.,~\citet{ji2009accelerated} and \citet{liu2009multi}.} This framework is generally applicable for many optimization schemes, such as proximal gradient methods~\citep{ji2009accelerated,liu2009multi}, alternating methods~\citep{argyriou2007multi} and Frank-Wolfe methods~\citep{jaggi2013revisiting}.

{\color{blue}Note that we mainly provided theoretical and experimental results for the $\W\W\trans$ type of covariance matrix. Nonetheless, the $\W\trans\W$ type of covariance matrix can be regarded as a natural alternative, since it is successfully used by \citet{zhang2010convex} (as a non-private method), \citet{gupta2016differentially} (as a differentially private method), and all the following MTL methods to learn relationship between tasks (see, e.g., the task relation learning approaches introduced by \citet{zhang2017survey} in Section 2.4 of their survey on MTL). Therefore, we included it in our framework. }
 
  
{\color{blue}
\begin{remark}
In Algorithm \ref{alg:MP-MTL}, a curator who collects models and performs centralized transfer just needs to run Step 4-6 and does not need to collect the datasets $(\X^m,\y^m)$, which are only used in STL algorithms.
\end{remark}
}
 
  

\begin{algorithm} [htb]
\caption{MP-MTL framework}
\label{alg:MP-MTL}{\small
\begin{algorithmic}[1]
\REQUIRE{Datasets $(\X^m,\y^m) = \{(\X_1,\y_1),\ldots,(\X_m,\y_m)\}$, where $\forall i\in[m], \ \X_i\in \mathbb{R}^{n_i \times d}$ and $\y_i\in \mathbb{R}^{n_i \times 1}$. Privacy loss $\epsilon , \delta  \geq 0$. Number of iterations $T$. Initial shared information matrix $\M^{(0)}$. Initial task models $\W^{(0)}$, which can be acquired via arbitrary STL methods.}
\ENSURE{$\widehat{\W}^{(1:T)}$ .}
\STATE Set $\{\epsilon_t\}$ such that {\color{blue} $CB(\{\epsilon_t\},\delta)\leq \epsilon$, where $CB(\{\epsilon_t\},\delta)$ is the composition bound of $\{\epsilon_t\}$.}
%\STATE   Normalize $\X^m$ to let the $\ell_2$ norm of each data point to be $1$.\\
\FOR{$t=1:T$}
{\color{blue}
\STATE Norm clipping: $\tilde{\w}_i^{(t-1)} = {\w}_i^{(t-1)}/\max(1,\frac{\|{\w}_i^{(t-1)}\|_2}{K})$, for all $i\in[m]$. Let $\widehat{\W}^{(0)} = \widetilde{\W}^{(0)}$.
}
\STATE  $\widetilde{\SSigma}^{(t)} = \widetilde{\W}^{(t-1)}(\widetilde{\W}^{(t-1)})\trans$ (or $\widetilde{\SSigma}^{(t)} = (\widetilde{\W}^{(t-1)})\trans\widetilde{\W}^{(t-1)}$).\label{eq:proximal_op_start}\\
\STATE  $\SSigma^{(t)} = \widetilde{\SSigma}^{(t)} + \E$, where $\E\sim W_d(d+1,\frac{K^2}{2\epsilon_t}\I_d)$ (or $\E\sim W_m(m+1,\frac{K^2}{2\epsilon_t}\I_m)$) is a sample from the Wishart distribution, $\I_d$ denotes the $d\times d$ identity matrix, and $\mbox{diag}(\cdot)$ transforms a vector into a diagonal matrix. \label{eq:add_wishart}\\
\STATE Perform an arbitrary mapping $f:\SSigma^{(1:t)}\rightarrow \M^{(t)}$, e.g., take the diagonal elements of $\SSigma^{(t)}$ or the singular value decomposition of $\SSigma^{(t)}$. \label{eq:proximal_op_end}\\
\STATE $\hat{\w}_i^{(t)}= \calA_{\mbox{st},i}(\M^{(t)}, \tilde{\w}_i^{(0:t-1)},\X_i,\y_i)$, for all $i\in[m]$, where $\calA_{\mbox{st},i}$ is an arbitrary STL algorithm for the $i$-th task and the $\tilde{\w}_i^{(0:t-1)}$ are used for initialization. \label{eq:STL_general} \\
\STATE Set the input for the next iteration: $\W^{(t)} = \widehat{\W}^{(t)}$.
\ENDFOR
\end{algorithmic}}
\end{algorithm}

\subsection{Instantiations of the MP-MTL Framework}
In this section, we instantiate our MP-MTL framework described in Algorithm \ref{alg:MP-MTL} by approximating the \emph{proximal gradient descent methods} presented by~\citet{ji2009accelerated} and~\citet{liu2009multi} for the \emph{trace-norm-regularized MTL problem} and the \emph{group-$\ell_1$-regularized MTL problem}, respectively.
{\color{blue}Both proximal gradient descent methods solve the respective MTL problems by alternatively perform a proximal operator step and a gradient decent step. Taking the \emph{trace-norm-regularized MTL problem} as an example, the loss function, $\sum_i\calL_i$, is minimized by the gradient decent steps, while the regularization term, the trace-norm, is minimized by the proximal operator steps. The proximal operator minimizes the regularization term, keeping the variable near the result of a previous gradient decent step. 
Specifically, we instantiate Steps 4-7 of Algorithm \ref{alg:MP-MTL} by approximating a proximal gradient descent step, i.e., first performing a proximal operator step and then taking a gradient decent step. It is similar for the \emph{group-$\ell_1$-regularized MTL problem}. The difference is in the instantiations of Step 6 of Algorithm \ref{alg:MP-MTL}, because different regularization terms leads to different optimal solutions of proximal operators. Note that both instantiations use the $\W\W\trans$ type of covariance matrix, which is required by the optimal solutions~\citep{ji2009accelerated,liu2009multi}. }  



First, we instantiate the MP-MTL framework for the \emph{trace-norm-regularized MTL problem}, as shown in Algorithm \ref{alg:MP-MTL-LR}. Generally speaking, the algorithm uses an accelerated proximal gradient method. Steps \ref{eq:prox_start_LR}-\ref{eq:feature_tran-LR} approximate the following proximal operator~\citep{ji2009accelerated}:
\begin{align}\label{eq:proximal_op_LR}
\widehat{\W}^{(t-1)} = \arg\min_{\W} \frac{1}{2\eta}\|\W - \widetilde{\W}^{(t-1)}\|_F^2 + \lambda\|\W\|_* ,
\end{align}
{\color{blue}where $\widetilde{\W}^{(t-1)}$ can be regarded as the result of the gradient decent step in the previous iteration, assuming $K$ is sufficiently large. In detail, Steps 6-8 of Algorithm \ref{alg:MP-MTL-LR} instantiate Step 6 of Algorithm \ref{alg:MP-MTL} by constructing a projection matrix $\M^{(t)} = \U\S_{\eta\lambda}\U\trans$ from the result of singular vector decomposition of the perturbed covariance matrix. Steps 9-11 of Algorithm \ref{alg:MP-MTL-LR} instantiate Step 7 of Algorithm \ref{alg:MP-MTL} by first projecting the models (in Step 9) then performing accelerated gradient descent.}
  
{
\begin{figure}[!t]\small
\centering
\subfigure[Before MTL]{\includegraphics[width=1.1in]{lowrank_before}} %diffk_simu_nmseg_1
\subfigure[After MTL with model leakage]{\includegraphics[width=1.1in]{lowrank_after}} %diffk_simu_aauc_1
\subfigure[After MTL with model protection]{\includegraphics[width=1.1in]{lowrank_after_add_noise}} %diffk_simu_aauc_1
\caption{Examples of model leakage and model protection, showing model matrices, where columns correspond to tasks and rows correspond to features. Columns shown have been divided by their respective $\ell_2$ norms.}\label{fig:privacy_leakage}
\end{figure}
}

We provide a running example for model leakage and model protection under different settings of Algorithm \ref{alg:MP-MTL-LR}, as shown in Fig.~\ref{fig:privacy_leakage}. {\color{blue} We generate models for $m=10$ tasks, respectively, in which the data dimension $d=5$. The 10-th task, the right-most one, is an anomaly task that requires privacy protection. In Fig.~\ref{fig:privacy_leakage} (a), the matrix denoted by $\W^{(0)}$ is firstly generated from i.i.d. uniform distribution $\mathcal{U}(0,1)$. Then the right-most column is multiplied by $100$. For MTL with model leakage, we run Algorithm \ref{alg:MP-MTL-LR}, taking $T=1, \eta=1,\epsilon_1 = \epsilon = 1e40, \delta = 0, K = 100\sqrt{5}$ and $\lambda = 50$. It can be regarded that the noise matrix $\E$ is not added, since $\epsilon \gg 1$. The output model matrix $\widehat{\W}^{(1)}$ is shown in Fig.~\ref{fig:privacy_leakage} (b), in which the 10-th task results in significantly influences on the parameters of other models: other models' parameters are similar to those of the 10-th task, e.g., for each task, the first feature is the biggest, and the fifth feature is the smallest. For MTL with model protection, we run Algorithm \ref{alg:MP-MTL-LR} with the same setting as above except that we set $\epsilon_1 = \epsilon = 0.1$. The output model matrix $\widehat{\W}^{(1)}$ is shown in Fig.~\ref{fig:privacy_leakage} (c), in which the influences from the 10-th task are not significant: other models' parameters are not similar to those of the 10-th task. Meanwhile, for $\W^{(0)}$ shown in Fig.~\ref{fig:privacy_leakage} (a), for tasks 1-9, the $\ell_2$ norms of the second and the fifth rows are of the two largest ones, which are significantly shown in Fig.~\ref{fig:privacy_leakage} (c). This means it is a shared information between tasks to use the second and the fifth features, which is successfully extracted by the MTL method with model protection.}


%We notice that the update rule proposed by~\citet{ji2009accelerated} for the parameter matrix $\W$ can be viewed as a recursive two-step procedure. The first step is to apply the gradient descent procedure to the prediction loss with respect to the model parameters, which are evaluated on each independent task. The second step is to obtain the parameters using the proximal operator induced by the regularizer. Concretely, the update rule involves the singular value decomposition (SVD): $\U\S\V = \widetilde{\W}=\W-\eta\nabla\W$, where $\eta$ denotes the step size and $\nabla\W$ denotes the gradient. Given $\U$ and $\S$, the computation for $\V$ can also be regarded as an STL learning algorithm because the $i$-th column of $\V$ is only related to $\w_i$; $\v_i =  \S^{\dag}\U\trans\w_i$ for all $i\in[m]$, where $(\cdot)^{\dag}$ denotes the Moore-Penrose inverse. Furthermore, $\U$ and $\S$ can be acquired from the SVD of the covariance matrix $\U\S^2\U = \widetilde{\W}\widetilde{\W}\trans$. As such, if the step size $\eta$ is fixed, information sharing occurs only when performing the SVD of $\widetilde{\W}\widetilde{\W}\trans$, which requires protection. Such procedure is described in Algorithm \ref{alg:MP-MTL-LR}.

\begin{algorithm} [htb]
\caption{MP-MTL Low-Rank Estimator}
\label{alg:MP-MTL-LR}{\small
\begin{algorithmic}[1]
\REQUIRE{Datasets $(\X^m,\y^m) = \{(\X_1,\y_1),\ldots,(\X_m,\y_m)\}$, where $\forall i\in[m], \ \X_i\in \mathbb{R}^{n_i \times d}$ and $\y_i\in \mathbb{R}^{n_i \times 1}$. Privacy loss $\epsilon , \delta  \geq 0$. Number of iterations $T$. Step size $\eta$. Regularization parameter $\lambda>0$. Norm clipping parameter $K>0$. Acceleration parameters $\{\beta_t\}$. Initial task models $\W^{(0)}$.}
\ENSURE{$\widehat{\W}^{(1:T)}$ .}
\STATE Set $\{\epsilon_t\}$ such that {\color{blue} $CB(\{\epsilon_t\},\delta)\leq \epsilon$, where $CB(\{\epsilon_t\},\delta)$ is the composition bound of $\{\epsilon_t\}$.}
%\STATE Normalize $\X^m$ to let the $\ell_2$ norm of each data point to be $1$.\\
\FOR{$t=1:T$}
\STATE Norm clipping: $\tilde{\w}_i^{(t-1)} = {\w}_i^{(t-1)}/\max(1,\frac{\|{\w}_i^{(t-1)}\|_2}{K})$, for all $i\in[m]$. Let $\widehat{\W}^{(0)} = \widetilde{\W}^{(0)}$.
\STATE {\color{blue} $\widetilde{\SSigma}^{(t)} = \widetilde{\W}^{(t-1)}(\widetilde{\W}^{(t-1)})\trans$.}\label{eq:prox_start_LR}\\
\STATE  $\SSigma^{(t)} = \widetilde{\SSigma}^{(t)} + \E$, where $\E\sim W_d(d+1,\frac{K^2}{2\epsilon_t}\I_d)$ is a sample from the Wishart distribution.\\
%\IF{$t<t_0$}\label{eq:theta_history-LR}
%\STATE  $\bar{\SSigma}^{(t)} = \SSigma^{(t)} $.
%\ELSE
%\STATE  Average the shared information:
%\begin{equation}\label{eq:mean_LR}
%\bar{\SSigma}^{(t)} = \frac{1}{t-t_0+1}\sum_{t'=t_0}^{t}\SSigma^{(t')}.
%\end{equation}
%\ENDIF
\STATE  Perform singular vector decomposition: $\U\LLambda\U\trans =  {\SSigma}^{(t)}$.\label{eq:trans_LR} %Let $\S$ be a diagonal matrix and $\S_{ii} = \sqrt{\LLambda_{ii}}$ for $i=1,\ldots,\min\{d,m\}$.\label{eq:trans_LR}
\STATE  Let $  \S_{\eta\lambda} $ be a diagonal matrix, and let $\S_{\eta\lambda,ii} = \max\{0, 1- \eta\lambda/\sqrt{\LLambda_{ii}} \}$, for $i=1,\ldots,\min\{d,m\}$.\\
%\STATE  Let $\v_i =   \U\trans\w_i^{(t-1)}$ for all $i\in[m]$, where $(\cdot)^{\dag}$ denotes the Moore-Penrose inverse.\\
\STATE {\color{blue}$\M^{(t)} = \U\S_{\eta\lambda}\U\trans$.}
\STATE  Let $ \hat{\w}_i^{(t)} = \M^{(t)}\tilde{\w}_i^{(t-1)}$, for all $i\in[m]$.\label{eq:feature_tran-LR}\\
\STATE  {Let $ {\z}_i^{(t)} =   \hat{\w}_i^{(t)} + \beta_t (\hat{\w}_i^{(t)} - \hat{\w}_i^{(t-1)})$, for all $i\in[m]$.}\label{eq:acc-LR} \\
\STATE  Let ${\w}_i^{(t)} = {\z}_i^{(t)} - \eta \frac{\partial \calL_i(\X_i{\z}_i^{(t)},\y_i)}{\partial {\z}_i^{(t)}}$, for all $i\in[m]$. \label{eq:gd-LR}\\
%\STATE Set the input for the next iteration: $\W^{(t)} = \widehat{\W}^{(t)}$.
\ENDFOR
\end{algorithmic}}
\end{algorithm}


Second, we instantiate the MP-MTL framework for the \emph{group-$\ell_1$-regularized MTL problem} defined in  \eqref{eq:MTL_L21}, as shown in Algorithm \ref{alg:MP-MTL-GS}. Steps \ref{eq:prox_start_GS}-\ref{eq:feature_select} approximate the following proximal operator~\citep{liu2009multi}:
\begin{align}\label{eq:proximal_op_GS}
\widehat{\W}^{(t-1)} = \arg\min_{\W} \frac{1}{2\eta}\|\W - \widetilde{\W}^{(t-1)}\|_F^2 + \lambda\|\W\|_{2,1}.
\end{align}
{\color{blue}The only difference between Algorithm \ref{alg:MP-MTL-GS} and Algorithm \ref{alg:MP-MTL-LR} is how to obtain the projection matrix $\M^{(t)}$ for models; see the difference between Steps 6-8 of Algorithm \ref{alg:MP-MTL-LR} and Steps 6-7 of Algorithm \ref{alg:MP-MTL-GS}. Since Algorithm \ref{alg:MP-MTL-GS} minimize the group-sparse penalty, it only focuses on the diagonal elements of the perturbed covariance matrix.
}
 

The bounds of errors from approximating the proximal operators are provided in Section \ref{sec:utility}.


%Then, we instantiate the MP-MTL framework for Problem \eqref{eq:MTL_L21}, the group-sparse case. We notice that the solution process proposed by~\citet{liu2009multi} can also be viewed as the aforementioned recursive two-step procedure. Concretely, the update rule of the parameter matrix $\W$ in the following given the $\ell_2$ norms of the rows of $\widetilde{\W}=\W-\eta\nabla\W$ can be regarded as an STL learning algorithm:
%\begin{align*}
% \hat{\w}^j = \max\{0, 1 -  \eta\lambda/ \|\tilde{\w}^j\|_2 \}  \tilde{\w}^j,
%\end{align*}
%because there are no interactions between the tasks if the $\ell_2$ norms of the rows of $\widetilde{\W}$ are given, where $\hat{\w}^j$ and $\tilde{\w}^j$ are the $j$-th row of $\widehat{\W}$ and $\widetilde{\W}$, respectively. $\lambda$ is some prefixed regularization parameter.
%
%Furthermore, the $\ell_2$ norms of the rows of $\widetilde{\W}$ are only related to the diagonal elements of the covariance matrix $\widetilde{\W}\widetilde{\W}\trans$. As such, if the step size $\eta$ is fixed, the information sharing only occurs when acquiring the diagonal elements of $\widetilde{\W}\widetilde{\W}\trans$, which needs protection. This procedure is described in Algorithm \ref{alg:MP-MTL-GS}.

\begin{algorithm} [htb]
\caption{MP-MTL Group-Sparse Estimator}
\label{alg:MP-MTL-GS}{\small
\begin{algorithmic}[1]
\REQUIRE{Datasets $(\X^m,\y^m) = \{(\X_1,\y_1),\ldots,(\X_m,\y_m)\}$, where $\forall i\in[m], \ \X_i\in \mathbb{R}^{n_i \times d}$ and $\y_i\in \mathbb{R}^{n_i \times 1}$. Privacy loss $\epsilon , \delta  \geq 0$. Number of iterations $T$. Step size $\eta$. Regularization parameter $\lambda>0$. Norm clipping parameter $K>0$.
Acceleration parameters $\{\beta_t\}$. Initial task models $\W^{(0)}$.}
\ENSURE{$\widehat{\W}^{(1:T)}$ .}
\STATE Set $\{\epsilon_t\}$ such that {\color{blue} $CB(\{\epsilon_t\},\delta)\leq \epsilon$, where $CB(\{\epsilon_t\},\delta)$ is the composition bound of $\{\epsilon_t\}$.}
%\STATE Normalize $\X^m$ to let the $\ell_2$ norm of each data point to be $1$.\\
\FOR{$t=1:T$}
\STATE {Norm clipping: $\tilde{\w}_i^{(t-1)} = {\w}_i^{(t-1)}/\max(1,\frac{\|{\w}_i^{(t-1)}\|_2}{K})$, for all $i\in[m]$.} Let $\widehat{\W}^{(0)} = \widetilde{\W}^{(0)}$.
\STATE  $\widetilde{\SSigma}^{(t)} = \widetilde{\W}^{(t-1)}(\widetilde{\W}^{(t-1)})\trans$.\label{eq:prox_start_GS} \\
\STATE  $\SSigma^{(t)} = \widetilde{\SSigma}^{(t)} + \E$, where $\E\sim W_d(d+1,\frac{K^2}{2\epsilon_t}\I_d)$ is a sample of the Wishart distribution.\\
%\IF{$t<t_0$} \label{eq:theta_history}
%\STATE  $\bar{\SSigma}^{(t)} = \SSigma^{(t)} $.
%\ELSE
%\STATE  Average the shared information:
%\begin{equation}\label{eq:mean_GS}
%\bar{\SSigma}^{(t)} = \frac{1}{t-t_0+1}\sum_{t'=t_0}^{t}\SSigma^{(t')}.
%\end{equation}
%\ENDIF
\STATE  Let $  \S_{\eta\lambda} $ be a diagonal matrix, where for $i=1,\ldots,d$, $\S_{\eta\lambda,ii}  = \max\{0, 1 -  \eta\lambda/ \sqrt{|{\SSigma}_{ii}^{(t)}|} \}$. \label{eq:construct_Mt}
\STATE {\color{blue}$\M^{(t)} = \S_{\eta\lambda}$.}
\STATE  Let $\hat{\w}_i^{(t)}  =  \M^{(t)} \tilde{\w}_i^{(t-1)}$, for all $i\in[m]$.\label{eq:feature_select}\\
\STATE  {Let $ {\z}_i^{(t)} =   \hat{\w}_i^{(t)} + \beta_t (\hat{\w}_i^{(t)} - \hat{\w}_i^{(t-1)})$, for all $i\in[m]$.}\label{eq:acc_select} \\
\STATE  Let $ {\w}_i^{(t)} =  {\z}_i^{(t)} - \eta \frac{\partial \calL_i(\X_i {\z}_i^{(t)},\y_i)}{\partial  {\z}_i^{(t)}}$, for all $i\in[m]$. \label{eq:gd}
%\STATE Set the input for the next iteration: $\W^{(t)} = \widehat{\W}^{(t)}$.
\ENDFOR
\end{algorithmic}}
\end{algorithm}

%\begin{remark}
%In Algorithm \ref{alg:MP-MTL-LR} and Algorithm \ref{alg:MP-MTL-GS}, the algorithms are presented under a basic proximal gradient descent scheme for simplicity. Nesterov’s accelerated methods in~\citet{ji2009accelerated} and~\citet{liu2009multi} can also be used directly as long as the step size $\eta$ is fixed and sufficiently small (being small to pass the line search and being fixed to guarantee privacy) because the MP-MTL framework allows the use of $\W^{(0:t-1)}$ for STL algorithms (the \ref{eq:STL_general}-th step of Algorithm \ref{alg:MP-MTL}).
%\end{remark}

%We note that in Algorithm \ref{alg:MP-MTL-LR}, in each step, the normalized parameter matrix $\widetilde{\W}^{(t-1)}$ is only used to compute the feature transformation matrix $\U\S_{\eta\lambda}\U\trans$, while the feature transformation $\hat{\w}_i^{(t)} = (\U\S_{\eta\lambda}\U\trans)\w_i^{(t-1)}$ (for all $i\in[m]$) is applied to the unnormalized parameter matrix ${\W}^{(t-1)}$ for all $t\in[T]$. Similarly, in Algorithm \ref{alg:MP-MTL-GS}, in each $t$-th iteration, the normalized parameter matrix $\widetilde{\W}^{(t-1)}$ is only used to compute the feature transformation matrix $\S_{\eta\lambda}$, while the feature transformation is applied to the unnormalized parameter matrix ${\W}^{(t-1)}$ in the \ref{eq:feature_select}-th step of Algorithm \ref{alg:MP-MTL-GS} for all $t\in[T]$.

%We note that in \eqref{eq:mean_LR} and \eqref{eq:mean_GS}, averaged share information $\frac{1}{t-t_0+1}\sum_{t'=t_0}^{t}\SSigma^{(t')}$ is used for reduce the variance. Guaranteed by Lemma \ref{th:lem_post}, it is allowed to use $\SSigma^{(1:t)}$ in the MP-MTL framework (the \ref{eq:historical_theta}th step of Algorithm \ref{alg:MP-MTL}), thus such averaging release no additional sensitive information. Intuitively, it is because that $\SSigma^{(1:t)}$ are assumed known by potential adversaries who can also perform such averaging.
 
 We use the following result to show that under high noise level, our algorithms share no information between models but keep the models intact, and thus degrade to STL methods such that they do not underperform comparing with STL methods.

\begin{proposition}\label{th:prop_better_than_STL}
For Algorithm \ref{alg:MP-MTL-LR}, the projection matrix $\U\S_{\eta\lambda}\U\trans$ degrades to an identity matrix , thus the algorithm degrades to an STL algorithm with no random perturbation, if the smallest singular value of $\E$ satisfies $\sigma_d(\E)= C \lambda^2$ for sufficiently large $C>0$.

For Algorithm \ref{alg:MP-MTL-GS}, the projection matrix $\S_{\eta\lambda}$ degrades to an identity matrix, thus the algorithm degrades to an STL algorithm with no random perturbation, if the smallest diagonal element of $\E$ satisfies $\min_j\E_{jj}= C \lambda^2$ for sufficiently large $C>0$.
\end{proposition}


We also consider other complex MTL frameworks for instantiation. For example, \citet{gong2012robust},~\citet{chen2011integrating},~\citet{jalali2010dirty} and~\citet{chen2012learning} considered a decomposed parameter/model matrix for handling heterogeneities among tasks, e.g., detecting entry-wise outliers in the parameter matrix~\citep{jalali2010dirty,chen2012learning} and detecting anomalous tasks~\citep{gong2012robust,chen2011integrating}. These detection procedures are claimed to be beneficial for the knowledge sharing process in the case of heterogeneous tasks. Our MP-MTL framework can be naturally extended to such a model-decomposed setting because the additional procedures are still STL algorithms, and hence, the privacy loss will not increase; see the supplementary material for additional details.




\subsection{Privacy Guarantees}

{\color{blue}The following two results show that our proposed framework and two instantiate algorithms satisfy the privacy constraint defined in Definition \ref{th:df_MP-MTL-iter}.}
\begin{theorem}\label{th:th_MP-MTL}
Algorithm \ref{alg:MP-MTL} is an $(\epsilon,\delta)$ - MP-MTL algorithm.
\end{theorem}

\begin{corollary}\label{th:th_MP-MTL-LR}
Algorithm \ref{alg:MP-MTL-LR} and Algorithm \ref{alg:MP-MTL-GS} are $(\epsilon,\delta)$ - MP-MTL algorithms.
\end{corollary}
 

{
\subsection{Utility Analyses}\label{sec:utility}
{\color{blue}We directly build utility analyses for our instantiations, Algorithm \ref{alg:MP-MTL-LR} and \ref{alg:MP-MTL-GS}, instead of Algorithm \ref{alg:MP-MTL}, because (1) Algorithm \ref{alg:MP-MTL} is a framework and allows minimizing a variety of regularization terms and many optimization schemes. Specifically, Steps 6 and 7 of Algorithm \ref{alg:MP-MTL} include arbitrary mappings and arbitrary STL algorithms, respectively. Therefore, the analysis is not trivial and needs additional assumptions. (2) Algorithm \ref{alg:MP-MTL-LR} and \ref{alg:MP-MTL-GS} correspond to trace-norm and group-$\ell_1$-norm regularization, respectively, which correspond to two main-stream approaches of MTL. 

Our utility analyses are built upon the matrix perturbation error bounds of Wishart noise presented by~\citet{jiang2016wishart}, error bounds with arbitrary heterogeneous residues of inexact proximal-gradient descent presented by~\citet{schmidt2011convergence} and two optimal solutions for proximal operators presented by~\citet{ji2009accelerated} and~\citet{liu2009multi}, respectively.
 
The following parts of the utility analyses are novel:
(1) the derivations of approximation error bounds for both the proximal operators in \eqref{eq:proximal_op_LR} and \eqref{eq:proximal_op_GS};
(2) the derivations of run time and utility bounds, considering three cases of composition bounds of privacy budgets, two privacy-budget allocation strategies, two specific regularization terms,  both convex and strongly convex prediction loss functions, and both the basic and accelerated proximal-gradient methods, subject to the elaborate composition theorem of privacy;
(3) the optimizations of the utility bounds with respect to parameters of privacy-budget allocation strategies.

We have studied the utility bounds for three cases of the {\color{blue}composition bound of $\{\epsilon_t\}$ defined in \eqref{eq:set_eps}}. Here, we report the results for the following case, {\color{blue}because this case can provide the minimum bound for small values of privacy budgets $\{\epsilon_t\}$ and $\delta$, such as for $\epsilon + e\delta\leq 1$; see~\citet{kairouz2017composition}.}
\begin{align*}
 \epsilon = \sum_{t=1}^{T}\frac{(e^{\epsilon_t}-1)\epsilon_t}{(e^{\epsilon_t}+1)}
+\sqrt{\sum_{t=1}^{T}2\epsilon_t^2\log\biggl(e+\frac{\sqrt{\sum_{t=1}^{T}\epsilon_t^2}}{\delta}\biggr)}.
\end{align*}
The results for the other two cases {\color{blue}are similar} and can be found in the supplementary material.

}


{\color{blue}

First, we make some assumptions.
}

\noindent\textbf{\emph{\underline{Parameter space}}}. A bounded parameter space is assumed for model matrices:
\begin{align*}
  \mathcal{W} = \{\W\in\mathbb{R}^{d\times m}: \max_{i\in[m]}\|\w_i\|_2\leq K\},
\end{align*}
where $K$ is the norm clipping parameter.

\noindent\textbf{\emph{\underline{Properties of objective functions}}}. We consider the loss function $f(\W) = \frac{1}{m}\sum\nolimits_{i=1}^m\calL_i(\X_i\w_i,\y_i)$. We assume that $mf(\W)$ is convex and has an $L$-Lipschitz-continuous gradient (as defined in \citet{schmidt2011convergence}).
Let $\W_* = \arg\min_{\W} mf(\W) + \lambda g(\W)$, where $g(\cdot) = \|\cdot\|_*$ for Algorithm \ref{alg:MP-MTL-LR} and $g(\cdot) = \|\cdot\|_{2,1}$ for Algorithm \ref{alg:MP-MTL-GS}. Without loss of generality, we assume that $\W_*\in \mathcal{W}$ and $f(\widetilde{\W}^{(0)})-f(\W_*) = O(K^2Lm)$. We adopt the notation $q = \min\{d,m\}$.

\noindent\textbf{\emph{\underline{The number of tasks}}}.
The number of tasks are assumed sufficient as follows.
\begin{assumption}\label{th:asm_m}
For Algorithm \ref{alg:MP-MTL-LR}, assume that for sufficiently large $C>0$,
\begin{align*}
m > CK^2d^2\log^2(d) (\log(e+\epsilon/\sqrt{2}\delta)+2\epsilon)/\epsilon^2
.
\end{align*}
 

For Algorithm \ref{alg:MP-MTL-GS}, assume that for sufficiently large $C>0$,
\begin{align*}
m > \left.C\log(d) \sqrt{\log(e+\epsilon/\sqrt{2}\delta)+2\epsilon}\middle/\epsilon\right..
\end{align*}

\end{assumption}

{\color{blue}Then we present the results. Before utility bounds, we report two intermediate results: approximation error bounds for proximal operators with trace-norm (low-rank) and group-$\ell_1$ (group-sparse) penalties, respectively. Note that for both results, the noise matrix $\E$ is allowed arbitrary.}
 
\begin{lemma}[Low rank]\label{th:lem_LR_iter_t}
Consider Algorithm \ref{alg:MP-MTL-LR}. For $t\in[T]$, in the $t$-th iteration, let $\C = \widetilde{\W}^{(t-1)}$. Let $r_c = \mbox{rank}(\C)\leq q$ be the rank of $\C$. Suppose that there exists an index $k\leq q$ such that $\sigma_{k}(\C) > \eta\lambda$ and $\sigma_{k+1}(\C) \leq \eta\lambda.$
Assume that $2\sigma_1(\E)\leq \sqrt{\sigma_j(\C)}-\sqrt{\sigma_{j+1}(\C)}$ for $j \in [k]$.
Then, for any random matrix $\E\in \mathbb{R}^{d\times d}$, the following holds:
\begin{equation}\label{eq:bound_LR_iter_t}
\begin{split}
&\frac{1}{2\eta}\|\widehat{\W}^{(t)} - \C\|_F^2 + \lambda\|\widehat{\W}^{(t)}\|_*  \\
&  - \biggl\{\min_{\W} \frac{1}{2\eta}\|\W - \C\|_F^2 + \lambda\|\W\|_*\biggr\}\\
\leq&\frac{1}{\eta}\biggl(\frac{\sigma_1^2(\C)}{\eta\lambda}+ \sigma_1(\C)\biggl)\\
&\cdot\biggl[ \biggl(\frac{k^2}{
 \eta\lambda} + 2k \biggr) \sigma_1(\E)   + \max(0,r_c-k)\sqrt{\sigma_1(\E)}\biggr].
\end{split}
\end{equation}
\end{lemma}


\begin{lemma}[Group Sparse]\label{th:lem_GS_iter_t}
Consider Algorithm \ref{alg:MP-MTL-GS}. For $t\in[T]$, in the $t$-th iteration, let $\C = \widetilde{\W}^{(t-1)}$. Let the indices of non-zero rows of $\C$ be denoted by $\mathcal{I}_c = \{j:\C^j\neq \mathbf{0}\}$, and let $r_{c,s} = |\mathcal{I}_c| \leq d$. Let $\SSigma_0 = \C\C\trans$. Suppose that there exists an integer $k\leq d$ such that $\sum_{j=1}^{d}I(\sqrt{\SSigma_{jj,0}}\geq \eta\lambda) = k,$
%\begin{align*}
%\sum_{j=1}^{d}I(\sqrt{\SSigma_{jj,0}}\geq \eta\lambda) = k,
%\end{align*}
where $I(\cdot)$ is the indicator function.
Then, for any random matrix $\E\in \mathbb{R}^{d\times d}$, the following holds:
\begin{equation}\label{eq:bound_GS_iter_t}
\begin{split}
&\frac{1}{2\eta}\|\widehat{\W}^{(t)} - \C\|_F^2 + \lambda\|\widehat{\W}^{(t)}\|_{2,1}  \\
&  - \biggl\{\min_{\W} \frac{1}{2\eta}\|\W - \C\|_F^2 + \lambda\|\W\|_{2,1}\biggr\}\\
\leq&\frac{1}{\eta}\biggl[\frac{r_{c,s}}{ \eta\lambda}\biggl(\max_{j\in[d]}\|\C^j\|_{2}\biggr)^2+ \biggl(\max_{j\in[d]}\|\C^j\|_{2}\biggr)\biggl]\\
 &\cdot\biggl[ \frac{k}{2\eta\lambda} \max_{j\in[d]}|\E_{jj}|   + \max(0,r_{c,s}-k) \max_{j\in[d]}\sqrt{|\E_{jj}|}\biggr].
\end{split}
\end{equation}
\end{lemma}

We find that both the approximation error bounds depend on
$\sigma_1(\E)$ (note that $\max_{j}|\E_{jj}|\leq \sigma_1(\E) $).

{\color{blue}Note that Lemma \ref{th:lem_LR_iter_t} requires that $\eta\lambda$ needs to fall between the $k$-th and the $(k+1)$-th singular values on every iteration for the same $k$. Under Assumption \ref{th:asm_m} (the number of tasks is sufficiently large), and if the initial task models in $W^{(0)}$ are acquired via proper STL methods, there will always be significant margin between the $k$-th and the $(k+1)$-th singular values of the normalized model matrix $\C$ for the same $k$. Therefore, it is easy to satisfy the above requirement. It is similar for the requirement of $k$ in Lemma \ref{th:lem_GS_iter_t}.}


%By \eqref{eq:set_eps}, we study utility bounds for the following case.

%\emph{Case 1}: $\epsilon = \sum_{t=1}^{T}\epsilon_t$.
%
%\emph{Case 2}: $\epsilon = \sum_{t=1}^{T}\frac{(e^{\epsilon_t}-1)\epsilon_t}{(e^{\epsilon_t}+1)}
%+\sqrt{\sum_{t=1}^{T}2\epsilon_t^2\log\biggl(\frac{1}{\delta}\biggr)}$.
%
%\emph{Case 3}:

%$\epsilon = \sum_{t=1}^{T}\frac{(e^{\epsilon_t}-1)\epsilon_t}{(e^{\epsilon_t}+1)}
%+\sqrt{\sum_{t=1}^{T}2\epsilon_t^2\log\biggl(e+\frac{\sqrt{\sum_{t=1}^{T}\epsilon_t^2}}{\delta}\biggr)}$.

Now, we present guarantees regarding both utility and run time.
In the following, $\E$ is assumed to be a Wishart random matrix in each iteration. Privacy budgets $\{\epsilon_t\}$ are considered heterogeneous, i.e., different with respect to $t\in[T]$.

{\color{blue}
We consider two cases for the loss function $f(\W)$: convex and strongly convex. For each case, we report the results of both Algorithms \ref{alg:MP-MTL-LR} (the low-rank estimator) and \ref{alg:MP-MTL-GS} (the group-sparse estimator). For each algorithm, we present the results for both the basic and the accelerated proximal gradient descent methods.

}

For the convex case of the loss function $f(\W)$, we set $\epsilon_t =\Theta(t^{\alpha})$ for $\alpha\in \mathbb{R}$ and $t\in[T]$. In this case, denote by
\begin{align*}
   M_0= \left.{\sqrt{\log(e+\epsilon/\sqrt{2}\delta)+2\epsilon} }\middle/{ \sqrt{|2\alpha+1|}\epsilon}\right.,
\end{align*}
which is used for both Theorem \ref{th:th_bound_LR_main_convex} and \ref{th:th_bound_GS_main_convex}.

\begin{theorem}[Low rank - Convexity]\label{th:th_bound_LR_main_convex}
Consider Algorithm \ref{alg:MP-MTL-LR}. For an index $k\leq q$ that satisfies the conditions given in Lemma \ref{th:lem_LR_iter_t} for all $t\in[T]$, $\eta =1/L$, and $\lambda = \Theta(LK\sqrt{m} )$, assume that $\epsilon_t\leq 4Kk^2d(\log d)/q^2$ for $t\in[T]$. Denote by 
%$$M = M_0Kkd\log d/\sqrt{m}$$.
\begin{align*}
M = M_0Kkd\log d/\sqrt{m}.
\end{align*}
% \begin{align*}
%   M= \frac{Kkd\log d\sqrt{\log(e+\epsilon/\sqrt{2}\delta)+2\epsilon} }{ \sqrt{|2\alpha+1|} \sqrt{m}\epsilon}.
% \end{align*}
\noindent\textbf{No acceleration}: If we set $\beta_t = 0$ for $t\in [m]$, then if we also set $T=\Theta(((\alpha/2 - 1)^2/M)^{\phi(\alpha)}  )$
for $\mathcal{E} = f(\frac{1}{T}\sum_{t=1}^{T}\widehat{\W}^{(t)}) - f(\W_*)$, we have, with high probability, 
%$\mathcal{E}= O( K^2L(M/(\alpha/2 - 1)^2)^{\phi(\alpha)}  )$,
\begin{equation}\label{eq:bound_LR_main_basic_convex}
\mathcal{E}= O( K^2L(M/(\alpha/2 - 1)^2)^{\phi(\alpha)}  ),
\end{equation}
% \begin{equation}\label{eq:bound_LR_main_basic_convex}
% \begin{split}
% \mathcal{E}= O\biggl( K^2L\bigg[\frac{Kkd\log d\sqrt{\log(e+\epsilon/\sqrt{2}\delta)+2\epsilon} }{ (\alpha/2 - 1)^2\sqrt{|2\alpha+1|} \sqrt{m}\epsilon}
%  \biggl]^{\phi(\alpha)}  \biggr),
% \end{split}
% \end{equation}
where
\begin{equation}\label{eq:bound_LR_main_basic_convex_phi}
\begin{split}
\phi(\alpha) =
\left\{
  \begin{array}{ll}
    2/(2\alpha+1), &  {\alpha>2;} \\
    2/5, &  {-1/2<\alpha<2;} \\
    1/(2-\alpha), &  {\alpha<-1/2.}
  \end{array}
\right.
\end{split}
\end{equation}

\noindent\textbf{Use acceleration}: If we set $\beta_t = {(t-1)}/{(t+2)}$ for $t\in [m]$, then if we also set $T=\Theta(((\alpha/2 - 2)^2/M)^{\phi(\alpha)/2}  )$
% \begin{align*}
% &T=\Theta\biggl(\bigg[\frac{ (\alpha/2 - 2)^2\sqrt{|2\alpha+1|} \sqrt{m}\epsilon}{Kkd\log d\sqrt{\log(e+\epsilon/\sqrt{2}\delta)+2\epsilon} }
%  \biggl]^{\phi(\alpha)/2}  \biggr)
% \end{align*}
for $\mathcal{E} = f(\widehat{\W}^{(T)}) - f(\W_*)$, we have, with high probability, 
%$\mathcal{E}= O( K^2L(M/(\alpha/2 - 2)^2)^{\phi(\alpha)}  )$,
\begin{equation}\label{eq:bound_LR_main_acc_convex}
\mathcal{E}= O( K^2L(M/(\alpha/2 - 2)^2)^{\phi(\alpha)}  ),
\end{equation}
% \begin{equation}\label{eq:bound_LR_main_acc_convex}
% \begin{split}
% \mathcal{E}= O\biggl( K^2L\bigg[\frac{Kkd\log d\sqrt{\log(e+\epsilon/\sqrt{2}\delta)+2\epsilon} }{ (\alpha/2 - 2)^2\sqrt{|2\alpha+1|} \sqrt{m}\epsilon}
%  \biggl]^{\phi(\alpha)}  \biggr),
% \end{split}
% \end{equation}
where
\begin{equation}\label{eq:bound_LR_main_acc_convex_phi}
\begin{split}
\phi(\alpha) =
\left\{
  \begin{array}{ll}
    4/(2\alpha+1), &  {\alpha>4;} \\
    4/9, &  {-1/2<\alpha<4;} \\
    2/(4-\alpha), &  {\alpha<-1/2.}
  \end{array}
\right.
\end{split}
\end{equation}
\end{theorem}

\begin{theorem}[Group sparse - Convexity]\label{th:th_bound_GS_main_convex}
Consider Algorithm \ref{alg:MP-MTL-GS}. For an index $k\leq d$ that satisfies the condition given in Lemma \ref{th:lem_GS_iter_t} for all $t\in[T]$, $\eta =1/L$, and $\lambda = \Theta(LKd\sqrt{m} )$, assume that $\epsilon_t\leq {k^2\log(d)}/{4Kd(d-k)^2m}$ for $t\in[T]$. Denote by 
%$M = M_0k\log d/m$.
\begin{align*}
 M = M_0k\log d/m.
\end{align*}
% \begin{align*}
%   M= \frac{k\log d\sqrt{\log(e+\epsilon/\sqrt{2}\delta)+2\epsilon} }{ \sqrt{|2\alpha+1|} m\epsilon}.
% \end{align*}
\noindent\textbf{No acceleration}: If we set $\beta_t = 0$ for $t\in [m]$, then if we also set $T=\Theta(((\alpha/2 - 1)^2/M)^{\phi(\alpha)}  )$
% \begin{align*}
% &T=\Theta\biggl(\bigg[\frac{ (\alpha/2 - 1)^2\sqrt{|2\alpha+1|} m\epsilon}{k\log d\sqrt{\log(e+\epsilon/\sqrt{2}\delta)+2\epsilon} }
%  \biggl]^{\phi(\alpha)}  \biggr)
% \end{align*}
for $\mathcal{E} = f(\frac{1}{T}\sum_{t=1}^{T}\widehat{\W}^{(t)}) - f(\W_*)$, we have, with high probability, 
%$\mathcal{E}= O( K^2L(M/(\alpha/2 - 1)^2)^{\phi(\alpha)}  )$,
\begin{equation}\label{eq:bound_GS_main_basic_convex}
\mathcal{E}= O( K^2L(M/(\alpha/2 - 1)^2)^{\phi(\alpha)}  ),
\end{equation}
% \begin{equation}\label{eq:bound_GS_main_basic_convex}
% \begin{split}
% \mathcal{E}= O\biggl( K^2L\bigg[\frac{k\log d\sqrt{\log(e+\epsilon/\sqrt{2}\delta)+2\epsilon} }{ (\alpha/2 - 1)^2\sqrt{|2\alpha+1|} m\epsilon}
%  \biggl]^{\phi(\alpha)}  \biggr),
% \end{split}
% \end{equation}
where $\phi(\alpha)$ is defined in \eqref{eq:bound_LR_main_basic_convex_phi}.

\noindent\textbf{Use acceleration}: If we set $\beta_t = {(t-1)}/{(t+2)}$ for $t\in [m]$, then if we also set $T=\Theta(((\alpha/2 - 2)^2/M)^{\phi(\alpha)/2}  )$
% \begin{align*}
% &T=\Theta\biggl(\bigg[\frac{ (\alpha/2 - 2)^2\sqrt{|2\alpha+1|} m\epsilon}{k\log d\sqrt{\log(e+\epsilon/\sqrt{2}\delta)+2\epsilon} }
%  \biggl]^{\phi(\alpha)/2}  \biggr)
% \end{align*}
for $\mathcal{E} = f(\widehat{\W}^{(T)}) - f(\W_*)$, we have, with high probability, 
%$\mathcal{E}= O( K^2L(M/(\alpha/2 - 2)^2)^{\phi(\alpha)}  )$,
\begin{equation}\label{eq:bound_GS_main_acc_convex}
\mathcal{E}= O( K^2L(M/(\alpha/2 - 2)^2)^{\phi(\alpha)}  ),
\end{equation}
% \begin{equation}\label{eq:bound_GS_main_acc_convex}
% \begin{split}
% \mathcal{E}= O\biggl( K^2L\bigg[\frac{k\log d\sqrt{\log(e+\epsilon/\sqrt{2}\delta)+2\epsilon} }{ (\alpha/2 - 2)^2\sqrt{|2\alpha+1|} m\epsilon}
%  \biggl]^{\phi(\alpha)}  \biggr),
% \end{split}
% \end{equation}
where $\phi(\alpha)$ is defined in \eqref{eq:bound_LR_main_acc_convex_phi}.
\end{theorem}


Next, we assume that $mf(\W)$ is $\mu$-strongly convex and has an $L$-Lipschitz-continuous gradient, where $\mu<L$.
We set $\epsilon_t =\Theta(Q^{-t})$ for $Q>0$ and $t\in[T]$ for this case. In this case, denote by
\begin{align*}
   M'_0=   \left.{ \sqrt{\log(e+\epsilon/\sqrt{2}\delta)+2\epsilon}}\middle/{ \sqrt{|1-Q^2|}  \epsilon}\right.,
\end{align*}
which is used for both Theorem \ref{th:th_bound_LR_main_strong_convex} and \ref{th:th_bound_GS_main_strong_convex}.


\begin{theorem}[Low rank - Strong convexity]\label{th:th_bound_LR_main_strong_convex}
Consider Algorithm \ref{alg:MP-MTL-LR}. For an index $k\leq q$ that satisfies the conditions given in Lemma \ref{th:lem_LR_iter_t} for all $t\in[T]$, $\eta =1/L$, and $\lambda = \Theta(LK\sqrt{m} )$, assume that $\epsilon_t\leq 4Kk^2d(\log d)/q^2$ for $t\in[T]$. Denote by 
%$M = M'_0Kkd\log d/\sqrt{m}$.
\begin{align*}
M = M'_0Kkd\log d/\sqrt{m}.
\end{align*}
% \begin{align*}
%   M=   \frac{ Kkd\log d \sqrt{\log(e+\epsilon/\sqrt{2}\delta)+2\epsilon}}{ \sqrt{|1-Q^2|} \sqrt{m}\epsilon}.
% \end{align*}
\noindent\textbf{No acceleration}: If we set $\beta_t = 0$ for $t\in [m]$, then if we let $Q_0 = 1-\mu/L$ and set $T=\Theta(\log_{1/\psi(Q,Q_0^2)}((Q_0/\sqrt{Q} - 1)^2/M)  )$
% \begin{align*}
% &T=\Theta\biggl(\log_{1/\psi(Q,Q_0^2)}\biggl[  \frac{ (Q_0/\sqrt{Q} - 1)^2\sqrt{|1-Q^2|} \sqrt{m}\epsilon}{ Kkd\log d \sqrt{\log(e+\epsilon/\sqrt{2}\delta)+2\epsilon}}  \biggr] \biggr)
% \end{align*}
for $\mathcal{E} = \frac{1}{\sqrt{m}}\|\widehat{\W}^{(T)}-\W_*\|_F$, we have, with high probability, 
%$\mathcal{E}= O(K(M/(Q_0/\sqrt{Q} - 1)^2)^{\log_{\psi(Q,Q_0^2)}Q_0}) $,
\begin{equation}\label{eq:bound_LR_main_basic_strong_convex}
\mathcal{E}= O(K(M/(Q_0/\sqrt{Q} - 1)^2)^{\log_{\psi(Q,Q_0^2)}Q_0}) ,
\end{equation}
% \begin{equation}\label{eq:bound_LR_main_basic_strong_convex}
% \begin{split}
% \mathcal{E}= O\biggl( K\biggl[  \frac{ Kkd\log d \sqrt{\log(e+\epsilon/\sqrt{2}\delta)+2\epsilon}}{ (Q_0/\sqrt{Q} - 1)^2\sqrt{|1-Q^2|} \sqrt{m}\epsilon}\biggr]^{\log_{\psi(Q,Q_0^2)}Q_0}  \biggr),
% \end{split}
% \end{equation}
where for any $\widetilde{Q}\in(0,1)$,
\begin{equation}\label{eq:bound_LR_main_basic_strong_convex_psi}
\begin{split}
\psi(Q,\widetilde{Q}) =
\left\{
  \begin{array}{ll}
    Q, &  {0<Q<\widetilde{Q};} \\
    \widetilde{Q}, &  {\widetilde{Q}<Q<1;} \\
    \widetilde{Q}/Q, &  {Q>1.}
  \end{array}
\right.
\end{split}
\end{equation}

\noindent\textbf{Use acceleration}: If we set $\beta_t = {(1-\sqrt{\mu/L})}/{(1+\sqrt{\mu/L})}$ for $t\in [m]$, then if we let $Q'_0 = 1-\sqrt{\mu/L}$ and set $T=\Theta(\log_{1/\psi(Q,Q'_0)}((\sqrt{Q'_0}/\sqrt{Q} - 1)^2/M)  )$
% \begin{align*}
% &T=\Theta\biggl(\log_{1/\psi(Q,Q'_0)}\biggl[  \frac{ (\sqrt{Q'_0}/\sqrt{Q} - 1)^2\sqrt{|1-Q^2|} \sqrt{m}\epsilon}{ Kkd\log d \sqrt{\log(e+\epsilon/\sqrt{2}\delta)+2\epsilon}}  \biggr] \biggr)
% \end{align*}
for $\mathcal{E} = f(\widehat{\W}^{(T)}) - f(\W_*)$, we have, with high probability, 
%$\mathcal{E}= O(K(M/(\sqrt{Q'_0}/\sqrt{Q} - 1)^2)^{\log_{\psi(Q,Q'_0)}Q'_0}) $,
\begin{equation}\label{eq:bound_LR_main_acc_strong_convex}
\mathcal{E}= O(K(M/(\sqrt{Q'_0}/\sqrt{Q} - 1)^2)^{\log_{\psi(Q,Q'_0)}Q'_0}),
\end{equation}
% \begin{equation}\label{eq:bound_LR_main_acc_strong_convex}
% \begin{split}
% \mathcal{E}= O\biggl( K\biggl[  \frac{ Kkd\log d \sqrt{\log(e+\epsilon/\sqrt{2}\delta)+2\epsilon}}{ (\sqrt{Q'_0}/\sqrt{Q} - 1)^2\sqrt{|1-Q^2|} \sqrt{m}\epsilon}\biggr]^{\log_{\psi(Q,Q'_0)}Q'_0}  \biggr),
% \end{split}
% \end{equation}
where $\psi(\cdot,\cdot)$ is defined in \eqref{eq:bound_LR_main_basic_strong_convex_psi}.
\end{theorem}

\begin{theorem}[Group sparse - Strong convexity]\label{th:th_bound_GS_main_strong_convex}
Consider Algorithm \ref{alg:MP-MTL-GS}. For an index $k\leq d $ that satisfies the condition given in Lemma \ref{th:lem_GS_iter_t} for all $t\in[T]$, $\eta =1/L$, and $\lambda = \Theta(LKd\sqrt{m} )$, assume that $\epsilon_t\leq {k^2\log(d)}/{4Kd(d-k)^2m}$ for $t\in[T]$. Denote by 
%$M = M'_0k\log d/m$.
\begin{align*}
M = M'_0k\log d/m.
\end{align*}
% \begin{align*}
%   M=     \frac{ k\log d \sqrt{\log(e+\epsilon/\sqrt{2}\delta)+2\epsilon}}{ \sqrt{|1-Q^2|} m\epsilon}.
% \end{align*}
\noindent\textbf{No acceleration}: If we set $\beta_t = 0$ for $t\in [m]$, then if we let $Q_0 = 1-\mu/L$ and set $T=\Theta(\log_{1/\psi(Q,Q_0^2)}((Q_0/\sqrt{Q} - 1)^2/M)  )$
% \begin{align*}
% &T=\Theta\biggl(\log_{1/\psi(Q,Q_0^2)}\biggl[  \frac{ (Q_0/\sqrt{Q} - 1)^2\sqrt{|1-Q^2|} m\epsilon}{ k\log d \sqrt{\log(e+\epsilon/\sqrt{2}\delta)+2\epsilon}}  \biggr] \biggr)
% \end{align*}
for $\mathcal{E} = \frac{1}{\sqrt{m}}\|\widehat{\W}^{(T)}-\W_*\|_F$, we have, with high probability, 
%$\mathcal{E}= O(K(M/(Q_0/\sqrt{Q} - 1)^2)^{\log_{\psi(Q,Q_0^2)}Q_0}) $,
\begin{equation}\label{eq:bound_GS_main_basic_strong_convex}
\mathcal{E}= O(K(M/(Q_0/\sqrt{Q} - 1)^2)^{\log_{\psi(Q,Q_0^2)}Q_0}),
\end{equation}
% \begin{equation}\label{eq:bound_GS_main_basic_strong_convex}
% \begin{split}
% \mathcal{E}= O\biggl( K\biggl[  \frac{ k\log d \sqrt{\log(e+\epsilon/\sqrt{2}\delta)+2\epsilon}}{ (Q_0/\sqrt{Q} - 1)^2\sqrt{|1-Q^2|} m\epsilon}\biggr]^{\log_{\psi(Q,Q_0^2)}Q_0}  \biggr),
% \end{split}
% \end{equation}
where $\psi(\cdot,\cdot)$ is defined in \eqref{eq:bound_LR_main_basic_strong_convex_psi}.

\noindent\textbf{Use acceleration}: If we set $\beta_t = {(1-\sqrt{\mu/L})}/{(1+\sqrt{\mu/L})}$ for $t\in [m]$, then if we let $Q'_0 = 1-\sqrt{\mu/L}$ and set $T=\Theta(\log_{1/\psi(Q,Q'_0)}((\sqrt{Q'_0}/\sqrt{Q} - 1)^2/M)  )$
% \begin{align*}
% &T=\Theta\biggl(\log_{1/\psi(Q,Q'_0)}\biggl[  \frac{ (\sqrt{Q'_0}/\sqrt{Q} - 1)^2\sqrt{|1-Q^2|} m\epsilon}{ k\log d \sqrt{\log(e+\epsilon/\sqrt{2}\delta)+2\epsilon}}  \biggr] \biggr)
% \end{align*}
for $\mathcal{E} = f(\widehat{\W}^{(T)}) - f(\W_*)$, we have, with high probability, 
%$\mathcal{E}= O(K(M/(\sqrt{Q'_0}/\sqrt{Q} - 1)^2)^{\log_{\psi(Q,Q'_0)}Q'_0}) $,
\begin{equation}\label{eq:bound_GS_main_acc_strong_convex}
\mathcal{E}= O(K(M/(\sqrt{Q'_0}/\sqrt{Q} - 1)^2)^{\log_{\psi(Q,Q'_0)}Q'_0}),
\end{equation}
% \begin{equation}\label{eq:bound_GS_main_acc_strong_convex}
% \begin{split}
% \mathcal{E}= O\biggl( K\biggl[  \frac{ k\log d \sqrt{\log(e+\epsilon/\sqrt{2}\delta)+2\epsilon}}{ (\sqrt{Q'_0}/\sqrt{Q} - 1)^2\sqrt{|1-Q^2|} m\epsilon}\biggr]^{\log_{\psi(Q,Q'_0)}Q'_0}  \biggr),
% \end{split}
% \end{equation}
where $\psi(\cdot,\cdot)$ is defined in \eqref{eq:bound_LR_main_basic_strong_convex_psi}.
\end{theorem}



\subsection{Privacy Budget Allocation}\label{subsec:Budget}
{\color{blue}In this section, we optimize the utility bounds presented in Theorems \ref{th:th_bound_LR_main_convex}-\ref{th:th_bound_GS_main_strong_convex} with respect to $\alpha$ and $Q$, respectively, which results in respective optimized privacy-budget allocation strategies. Then we discuss the optimized results.}


\begin{theorem}\label{th:th_budget}
Consider Algorithm \ref{alg:MP-MTL-LR} and  Algorithm \ref{alg:MP-MTL-GS}.

For a \emph{convex} $f$, use Theorem \ref{th:th_bound_LR_main_convex} and Theorem \ref{th:th_bound_GS_main_convex}.

(1) \emph{No acceleration}: The bounds for low-rank and group-sparse estimators both reach their respective minima w.r.t. $\alpha$ at $\alpha = 0$. Meanwhile, $\phi(\alpha) = 2/5$.

(2) \emph{Use acceleration}: The bounds for low-rank and group-sparse estimators both reach their respective minima w.r.t. $\alpha$ at $\alpha = 2/5$. Meanwhile, $\phi(\alpha) = 4/9$.

For a \emph{strongly convex} $f$, use Theorem \ref{th:th_bound_LR_main_strong_convex} and Theorem \ref{th:th_bound_GS_main_strong_convex}.

(1) \emph{No acceleration}: The bounds for low-rank and group-sparse estimators both reach their respective minima w.r.t. $Q$ at $Q = Q_0^{2/5}$. Meanwhile, $\log_{\psi(Q,Q_0^2)}Q_0 = 1/2$.

(2) \emph{Use acceleration}: The bounds for low-rank and group-sparse estimators both reach their respective minima w.r.t. $Q$ at $Q = (Q'_0)^{1/5}$. Meanwhile, $\log_{\psi(Q,Q'_0)}Q'_0 = 1$.
\end{theorem}

Results corresponding to the optimized privacy-budget allocation strategies (with $\delta>0$) are summarized in Table \ref{tab:utility_results}, where the terms with respect to $K,L,k$, and $\sqrt{\log(e+\epsilon/\sqrt{2}\delta)+2\epsilon}$ are omitted, and the results associated with the setting $\epsilon = \sum_{t=1}^{T}\epsilon_t$ (and $\delta=0$) are also included, which provides $(\epsilon,0)$ - MP-MTL algorithms.

\setlength{\tabcolsep}{2pt}
\begin{table}[htbp]\small
  \centering
  \renewcommand{\multirowsetup}{\centering}
    \caption{Utility results.}\label{tab:utility_results}
  \begin{tabular}{c|c|c|c|c}
  \hline
     \hline
     & & &Low rank& Group sparse\\
     \hline
     \multirow{4}{*}{$\delta=0$}&\multirow{2}{1.6cm}{\footnotesize No Acceleration}&Convex& $\mathcal{O}((\frac{d\log(d)}{\sqrt{m}\epsilon})^{\frac{1}{3}})$ &$\mathcal{O}((\frac{\log(d)}{{m}\epsilon})^{\frac{1}{3}})$ \\
   \cline{3-5}
   &&Strong convex&$\mathcal{O}((\frac{d\log(d)}{\sqrt{m}\epsilon})^{\frac{1}{2}})$ &$\mathcal{O}((\frac{\log(d)}{{m}\epsilon})^{\frac{1}{2}})$ \\
   \cline{2-5}
    &\multirow{2}{1.6cm}{\footnotesize Use Acceleration}&Convex&$\mathcal{O}((\frac{d\log(d)}{\sqrt{m}\epsilon})^{\frac{2}{5}})$  & $\mathcal{O}((\frac{\log(d)}{{m}\epsilon})^{\frac{2}{5}})$\\
    \cline{3-5}
    &&Strong convex&$\mathcal{O}(\frac{d\log(d)}{\sqrt{m}\epsilon})$&$\mathcal{O}(\frac{\log(d)}{{m}\epsilon})$\\
   \hline
   \multirow{4}{*}{$\delta>0$}&\multirow{2}{1.6cm}{\footnotesize No Acceleration}&Convex& $\mathcal{O}((\frac{d\log(d)}{\sqrt{m}\epsilon})^{\frac{2}{5}})$ &$\mathcal{O}((\frac{\log(d)}{{m}\epsilon})^{\frac{2}{5}})$ \\
   \cline{3-5}
   &&Strong convex&$\mathcal{O}((\frac{d\log(d)}{\sqrt{m}\epsilon})^{\frac{1}{2}})$ &$\mathcal{O}((\frac{\log(d)}{{m}\epsilon})^{\frac{1}{2}})$ \\
    \cline{2-5}
    &\multirow{2}{1.6cm}{\footnotesize Use Acceleration}&Convex&$\mathcal{O}((\frac{d\log(d)}{\sqrt{m}\epsilon})^{\frac{4}{9}})$  & $\mathcal{O}((\frac{\log(d)}{{m}\epsilon})^{\frac{4}{9}})$\\
    \cline{3-5}
    &&Strong convex&$\mathcal{O}(\frac{d\log(d)}{\sqrt{m}\epsilon})$&$\mathcal{O}(\frac{\log(d)}{{m}\epsilon})$\\
   \hline
   \hline
  \end{tabular}
\end{table}

{\color{blue}We learn from Theorem \ref{th:th_budget} that (1) for all four settings, a non-decreasing series of $\{\epsilon_t\}$ results in a good utility bound, since the best $\alpha = 0, 2/5 \geq 0$ for $\epsilon_t=\Theta(t^{\alpha})$ and the best $Q = Q_0^{2/5}, (Q'_0)^{1/5} < 1$ for $\epsilon_t=\Theta(Q^{-t})$. Intuitively, this means adding non-increasing noises over iterations, which is reasonable since initial iterations may move quickly in the parameter space while the last iterations may only fine-tune the model by a little. (2) Both the strong-convexity condition and the acceleration strategy improve the utility bounds, since they both increase the powers of the bounds which are far less than $1$ under Assumption \ref{th:asm_m}.  (3) Setting $\alpha$ and $Q$ by the optimized values, respectively, we can observe that the acceleration strategy can improve run time, as shown in Claim \ref{claim:acc_runtime}.

\begin{claim}\label{claim:acc_runtime}
Assume Assumption \ref{th:asm_m}. Consider Theorem \ref{th:th_bound_LR_main_convex}-\ref{th:th_bound_GS_main_strong_convex} and set $\alpha$ and $Q$ by the optimized values in Theorem \ref{th:th_budget}, respectively. Assume $\mu/L<0.3819$. The values for $T$ are smaller using the acceleration strategy in comparison with those with no acceleration, respectively.
\end{claim}
 

  
   
}

Now, we introduce our concrete strategy in the following to set $\{\epsilon_t\}$ in both Algorithm \ref{alg:MP-MTL-LR} and  Algorithm \ref{alg:MP-MTL-GS}. We assume that $T$, $\epsilon$ and $\delta$ are given. {\color{blue}Note that this strategy is optimal if $\alpha$ and $Q$ are set according to the optimal settings stated by Theorem \ref{th:th_budget}.}

For a \emph{convex} $f$, if no acceleration is to be used, then set $\beta_t = 0$ for $t\in [m]$ and set $\alpha \in \mathbb{R}$ (e.g., $\alpha=0$); otherwise, set $\beta_t = {(t-1)}/{(t+2)}$ for $t\in [m]$ and set $\alpha \in \mathbb{R}$ (e.g., $\alpha = 2/5$). Then, for $t\in[T]$, let $\epsilon_t = \epsilon_0t^{\alpha}$ and find the largest $\epsilon_0$ that satisfies $CB(\{\epsilon_t\},\delta)\leq \epsilon$, where $CB(\{\epsilon_t\},\delta)$ is the composition bound of $\{\epsilon_t\}$ defined in \eqref{eq:set_eps}.

For a \emph{$\mu$-strongly convex} $mf(\W)$ with a known value of $\mu$ (e.g., $\frac{\mu}{2}\|\w_i\|_2^2$ is added to each $\mathcal{L}_i$), if no acceleration is to be used, then set $\beta_t = 0$ for $t\in [m]$ and set $Q > 0$ (e.g., $Q=(1-\mu/L)^{2/5}$, if $L$ is known); otherwise, if $L$ is known, set $\beta_t = {(1-\sqrt{\mu/L})}/{(1+\sqrt{\mu/L})}$ for $t\in [m]$ and set $Q>0$ (e.g., $Q=(1-\sqrt{\mu/L})^{1/5}$). Then, for $t\in[T]$, let $\epsilon_t = \epsilon_0Q^{-t}$ and find the largest $\epsilon_0$ that satisfies $CB(\{\epsilon_t\},\delta)\leq \epsilon$, where $CB(\{\epsilon_t\},\delta)$ is the composition bound of $\{\epsilon_t\}$ defined in \eqref{eq:set_eps}.


}

\subsection{Baseline MP-MTL constructed by IP-MTL}\label{subsec:SMC}

%{In contrast with the proposed model-protected MTL approach, privacy-preserving MTL algorithms that \emph{prevent a single data instance} for one task from leaking to other tasks can be regarded as \emph{Instance-Protected} MTL (IP-MTL) algorithms.} 
  
IP-MTL algorithms \emph{prevent a single data instance} for one task from leaking to other tasks, which are defined formally as follows. 

\begin{definition}[IP-MTL]\label{th:df_DP-MTL-iter}
Let $\calA$ be a randomized MTL algorithm with a number of iterations $T$. In the first iteration, $\calA$ performs the mapping $(\W^{(0)} \in\mathbb{R}^{d\times m},\calD^m)\rightarrow \theta_1\in \calC_1$, where $\theta_1$ includes $\widehat{\W}^{(1)} \in\mathbb{R}^{d\times m}$. For $t=2,\ldots,T$, in the $t$-th iteration, $\calA$ performs the mapping $(\W^{(t-1)} \in\mathbb{R}^{d\times m},\calD^m,\theta_1,\ldots,\theta_{t-1})\rightarrow \theta_t\in \calC_t$, where $\theta_t$ includes $\widehat{\W}^{(t)} \in\mathbb{R}^{d\times m}$. $\calA$ is an $(\epsilon,\delta)$ - \emph{IP-MTL} algorithm if for all $i\in[m]$ and for all neighboring datasets $\calD^m$ and $(\calD')^m$ that differ by a single data instance for the $i$-th task, the following holds for some constants $\epsilon,\delta\geq 0$ and for any set $\calS \subseteq \mathbb{R}^{d\times (m-1)\times T}$:

\begin{equation}\label{eq:DP_MTL-iter}
\begin{split}
\bbP( &  \hat{ \w}_{[-i]}^{(1:T)}  \in \calS  \mid \bigcap_{t=1}^T \calB_t = (\W^{(t-1)}, \calD^m, \ttheta_{1:t-1}) ) \\
\leq   &e^{\epsilon} \bbP(  \hat{ \w}_{[-i]}^{(1:T)} \in \calS \mid \bigcap_{t=1}^T \calB_t = ((\W')^{(t-1)}, (\calD')^m, \ttheta_{1:t-1})) \\
&+ \delta,
\end{split}
\end{equation}
where for all $t\in[T]$, $\calB_t$ denotes the input for the $t$-th iteration,
\begin{numcases}{\ttheta_{1:t-1} = }
\nonumber \emptyset, & $t=1$\\
\nonumber \theta_1,\theta_2,\cdots,\theta_{t-1}, & $t\geq2$,
\end{numcases}
and $(\W')^{(t-1)}$ is associated with the setting in which a single data instance for the $i$-th task has been replaced.
\end{definition}


As examples, the methods of \citet{pathak2010multiparty} and~\citet{gupta2016differentially} both fall into this category.  
\begin{proposition}\label{th:DP-MP-iter_example}
The methods of both \citet{pathak2010multiparty} and~\citet{gupta2016differentially} are IP-MTL algorithms with $T=1$ and $T\geq 1$, respectively.
\end{proposition}


Now we can construct baseline MP-MTL methods by IP-MTL methods using the result of Proposition \ref{th:prop_DP-MP-iter}: to guarantee an $(\epsilon,\delta)$ - MP-MTL algorithm, one can use an $(\epsilon/n,\delta/(n\exp(\epsilon))$ - IP-MTL algorithm.
\begin{proposition}\label{th:prop_DP-MP-iter}
For tasks' sample sizes $n_1,\ldots,n_m$, any $(\epsilon,\delta)$ - IP-MTL algorithm is a $(n\epsilon,n\exp(n\epsilon)\delta)$ - MP-MTL algorithm, where $n=\max_{i\in[m]}n_i$.
\end{proposition}
{\color{blue}The proof of Proposition \ref{th:prop_DP-MP-iter} can be found in the supplementary material, which directly follows the proof of the group privacy Lemma stated by Lemma 2.2 of~\citet{vadhan2016complexity}. Therefore, Proposition \ref{th:prop_DP-MP-iter} be regarded as the group privacy property of differential privacy applied to a ``group'' of the entire dataset for a single task. }
 

%{\color{blue}From Proposition \ref{th:prop_DP-MP-iter} we can learn that, it is limiting to directly enforce "group privacy" by IP-MTL to realize MP-MTL, since the privacy budgets are related to the maximum sample size of all the tasks, which will induce excessive noises to other tasks that have smaller sample sizes. This the reason that we aim to propose a more effective model-protected MTL method as an alternative.}

%Therefore, by Proposition \ref{th:prop_DP-MP-iter}, 

 

% \subsection{Tuning for Hyper-Parameters}
% The hyper-parameters, e.g., $\lambda$ in Problem \eqref{eq:MTL_L21} and \eqref{eq:MTL_Trace}, are assumed fixed so far. In real MTL application, they may be selected based on the data sets $(\X^m,\y^m)$. Since the selection may involve multiple tasks, the information of models of involved tasks may also be leaked into the hyper-parameters. Such consideration is similar as the parameter tuning issue discussed by~\citet{chaudhuri2011differentially}, where tuning hyper-parameters may loose privacy for single data instance.

% For the typical hyper-parameter tuning method that selecting the best model trained on the training data sets on the held out validation data sets, we can use the similar strategies proposed by~\citet{chaudhuri2011differentially} to tune hyper-parameters for our MP-MTL methods.

% Suggested by~\citet{chaudhuri2011differentially}, the first strategy is using a small data set which has already been public to tune hyper-parameters. It should be assumed that: 1) such data set exist; 2) the hyper-parameters tuned on the data set correspond to a good model for the private data set which is actually considered.

% Similar to the second strategy of~\citet{chaudhuri2011differentially} to separate data instances, our second strategy is to separate tasks, which is described in Algorithm \ref{alg:MP-MTL-hyper}. This final algorithm provides an end-to-end guarantee of differential privacy, and renders our MP-MTL procedure complete.

% \begin{algorithm} [htb]
% \caption{Hyper-parameter tuning for MP-MTL methods}
% \label{alg:MP-MTL-hyper}{\small
% \begin{algorithmic}[1]
% \REQUIRE{Data sets $(\X^m,\y^m) = \{(\X_1,\y_1),\ldots,(\X_m,\y_m)\}$, where $\forall i\in[m], \ \X_i\in \mathbb{R}^{n_i \times d}$ and $\y_i\in \mathbb{R}^{n_i \times 1}$. Privacy loss $\epsilon , \delta  \geq 0$. Number of iterations $T$. A series of hyper-parameters $\{\llambda_1,\ldots,\llambda_{k}\}$.}
% \ENSURE{$\widehat{\W}$.}
% \STATE Hold out part of training data as validation data for each task.
% \STATE Apply an specified $(\epsilon/2, \delta/2)$-Iterative MP-MTL algorithm (e.g., Algorithm \ref{alg:Iterative MP-MTL_by_MP-MTL}, \ref{alg:MP-MTL}, \ref{alg:MP-MTL-GS}, \ref{alg:MP-MTL-LR}, \ref{alg:MP-MTL-SMC}, and \ref{alg:MP-MTL-LR-SP}) with the number of iterations of $kT$. Use each of the hyper-parameters $\{\llambda_1,\ldots,\llambda_{k}\}$ for each consecutive $T$ iterations. Reset all the parameters to initial values in every $T$th iteration. Get $k$ groups of output $(\widehat{\W}_1^{(1:T)},\ldots,\widehat{\W}_k^{(1:T)})$.\\
% \FOR{$r=1:k$}
% \STATE Evaluate $z_r$ which is some evaluation score and made by $\widehat{\W}_{r}^{(1:T)}$ on the validation data. Lower score represents better model.\\
% \ENDFOR
% \STATE Set $\hat{r} = r$ with probability
% \begin{equation}\label{eq:MP-MTL-hyper}
%  p(\hat{r} = r) = \frac{\exp(-\epsilon z_r/2)}{\sum_{r=1}^{k}\exp(-\epsilon z_r/2)}.
% \end{equation}
% \STATE Apply the specified $(\epsilon/2, \delta/2)$-Iterative MP-MTL algorithm with hyper-parameter $\llambda_{\hat{r}}$ to get output $\widehat{\W}^{(1:T)}$.\\
% \end{algorithmic}}
% \end{algorithm}

% In Algorithm \ref{alg:MP-MTL-hyper}, for $r=1,\ldots,k$, $\llambda_r$ can include multiple hyper-parameters, such as $\lambda_1$ and $\lambda_2$ in Algorithm \ref{alg:MP-MTL-LR-SP}.
% %
% %We also note that in Algorithm \ref{alg:MP-MTL-hyper}, for $r=1,\ldots,k$, to apply an $(\epsilon, \delta)$ - Iterative MP-MTL algorithm, one should modify \eqref{eq:set_eps} as
% %\begin{equation*}
% %  \tilde{\epsilon} =  \sum_{t=1}^{T}\epsilon_t.
% %\end{equation*}

% The following two corollaries follow from Theorem 26 and 27 of~\citet{chaudhuri2011differentially}.
% \begin{corollary}\label{th:th_MP-MTL-hyper-privacy}
% Use Theorem 26 of~\citet{chaudhuri2011differentially}. Algorithm \ref{alg:MP-MTL-hyper} is an $(\epsilon,\delta)$ - Iterative MP-MTL algorithm.
% \end{corollary}

% \begin{corollary}\label{th:th_MP-MTL-hyper-utility}
% Use Theorem 27 of~\citet{chaudhuri2011differentially}. Let $z_{\min} = \min_i z_i$, and let $z$ be the evaluation score made on the $(k+1)$th group by $\widehat{\W}^{(1:T)}$. Then, with probability $1- \gamma$,
% \begin{equation*}
%  z\leq z_{\min} + \frac{2\log(k/\gamma)}{\epsilon}.
% \end{equation*}
% \end{corollary}




==> related_work.tex <==
%!TEX root = MultitaskDP.tex

%\section{Related Work}\label{sec:related}
%
%Few privacy-preserving multi-task learning approaches have been proposed~\citep{mathew2012distributed,baytas2016asynchronous,pathak2010multiparty,shokri2015privacy,gupta2016differentially} . However, such approaches only attempt to ensure the security of data instances rather than of models/predictors.
%
%A typical direction of research is distributed learning~\citep{mathew2012distributed,baytas2016asynchronous}, where the datasets of tasks are located distributively. The local models of tasks are trained independently using their own dataset before being aggregated and injected with useful knowledge shared across tasks. Such a procedure is typically non-private from the differential privacy point of view because no perturbation is added; hence, potential attackers may obtain information of all the tasks based on the information of only one task. Another typical direction of research has been to take differential privacy into account. Pathak et al.~\citep{pathak2010multiparty} proposed a differentially private multi-task logistic regression scheme to first train local models distributively and then average the decision vectors of the tasks after adding noise based on the output perturbation method of~\citep{dwork2006calibrating}. However, because it only performs averaging, the ability to cover the different relatedness of tasks is limited. Gupta et al.~\citep{gupta2016differentially} proposed a scheme to transform multi-task relationship learning (MTRL)~\citep{zhang2012convex} into a differentially private version, where the output perturbation method is adopted as well. However, they neglected considering the accumulated effect of privacy due to the iterative procedure of their algorithm. Moreover, on their synthetic datasets, their private MTL methods even underperform the non-private single-task learning methods (which can guarantee optimal privacy against leaking information across tasks), which may make it unnecessary to use their private MTL methods. Both works attempted to protect a single data instance instead of the predictor/model of each task, and they added noise directly to the predictors, which is not necessary for the purpose of avoiding leaking information across tasks and may induce excess noise and thus jeopardize the utility of the algorithms.


%Both works has two common drawbacks: 1) they add noise directly on the predictors, which is not necessary for the purpose of avoid leaking information across tasks and will induce excess noise to jeopardize the utility of algorithm; 2) their methods to transform MTL methods to their differentially private versions are restricted to specific MTL methods, the potential generalization to other MTL methods is limited.



%We introduce existing research on multi-task learning and differential privacy in this section.

%\subsection{Multi-Task Learning}

%Multi-task learning is a type of transfer learning algorithm that performs inductive transfer among a set of related machine learning tasks, where a learning task can be either classification, regression or clustering. By comparison, single-task learning (STL) is a type of algorithm that learn each task independently. The key to multi-task learning is to connect the tasks via a shared representation, which in turn benefits the tasks to be learned. Each shared representation encodes certain assumptions on the task relatedness.

%There are extensive multi-task learning studies on linear models using regularized approaches. Linear models are simple yet powerful in that flexible regularization can be designed according to desired structures and assumptions. Moreover, the point estimation of linear models often yields efficient optimization algorithms. The key to multi-task learning is to connect the tasks via a shared representation, which in turn benefits the tasks to be learned. Each shared representation encodes certain assumptions on the task relatedness. In many real-world applications, we can assume that there are some latent variables, and the tasks are related via the latent variables.

%Among the regularized linear MTL models, there are many different assumptions on how tasks are related.



%\subsection{Differential privacy  }

%Differential privacy~\citep{dwork2011firm,dwork2006calibrating,dwork2014algorithmic} represents a strong standard for privacy guarantees for algorithms, where one wishes to avoid potential attackers acquiring the information of any element of the input dataset based on a change in the output distribution.

%Differential private learning can be achieved by introducing some perturbation in the original learning system to the (1) input data~\citep{Li2014,BCDKMT07,xiao2011differential}, (2) model parameters~\citep{XWG10,FS10,Ji2013, Ji2014a,chaudhuri2008privacy}, (3)  objective function~\citep{CMS11,Zhang2012}, or (4) optimization process~\citep{Song2013,wang2015privacy}.


%Li et al.~\citep{Li2014} proposed a framework to compute a differentially private copula function from input data and sample synthetic data from the function to capture the dependencies implicit in the dataset. Barak et al.~\citep{BCDKMT07} transformed the input data into a frequency matrix, which was converted into the Fourier domain to introduce Laplacian noise. Xiao et al.~\citep{xiao2011differential} proposed a Privelet method by applying a wavelet transform to the original histogram and then adding noise. These models generate differentially private data that can be used for any learning model. There are also input perturbation models customized for learning tasks, for example, classification. Noman et al.~\citep{XWG10} proposed a top-down decision-tree-based approach to disseminate differentially private data. Friedman and Schuster~\citep{FS10} developed another model to generate differentially private data for decision trees. Ji et al.~\citep{Ji2013, Ji2014a} developed an importance weighting model to generate differentially private data for SVM and logistic regression.
%Another technique is to add noise directly to the outcomes. For parametric models, Chaudhuri et al.~\citep{chaudhuri2008privacy} proposed a parameter perturbation approach based on the sensitivity of the parameters. However, this approach may introduce too much noise. They also developed an object perturbation technique~\citep{CMS11} that guarantees that the outcomes of the optimization are differentially private. Using this technique, Zhang et al.~\citep{Zhang2012} conducted differentially private linear regression and logistic regression. The objective perturbation mechanism imposes convexity and differentiability requirements on the loss and regularizer, which cannot always be met.
%Another approach is to perturb the optimization process. Song et al.~\citep{Song2013} developed a mechanism for stochastic gradient descent with differentially private updates. Wang et al.~\citep{wang2015privacy} recently developed a posterior sampling technique to preserve differential privacy with minor changes to the algorithmic procedures.





\section{Preliminaries and the Proposed Problem}\label{sec:pre}

%We introduce the background on MTL problems and useful tools for differential privacy in this section.

{
In this section, we first introduce the background on MTL problems and then introduce the definition of model-protection problems for MTL.
}

The notations and symbols that will be used throughout the paper are summarized in Table \ref{tab:notations}.

\begin{table}[htbp]
\centering
\caption{Notations and Symbols}
\label{tab:notations}
{\small
\begin{tabular}{l|p{20em}}
\hline\hline $[k]$& the index set $\{1,2,\cdots,k\}$\\
\hline
$[-i]$& the index set with index $i$ removed\\
\hline $\|\cdot\|_{*}$& the trace norm of a matrix (sum of the singular values of the matrix)\\
\hline $\|\cdot\|_{2,1}$& the $\ell_{2,1}$ norm of a matrix (sum of the $\ell_2$ norms of the row vectors of the matrix)\\
\hline ${\rm tr(\cdot)}$& the trace of a matrix (sum of the diagonal elements of the matrix)\\
\hline $\sigma_j(\cdot)$& the $j$-th largest singular value of a matrix, $j\in[m]$\\
%\hline $ c=\rm{STL}(a,b)$& the trace of a matrix (sum of the diagonal elements in the matrix)\\
%\hline $\|\cdot\|_{1}$& $\ell_1$-norm of a matrix (sum of the absolute value of all elements in the matrix)\\
\hline\hline
\end{tabular}}
\end{table}


Extensive MTL studies have been conducted on linear models using regularized approaches.
The basic MTL algorithm that we will consider is as follows:
\begin{equation}\label{eq:MTL_ONE}
\widehat{\W} = \arg\min_{\W} \sum\nolimits_{i=1}^m\calL_i(\X_i\w_i,\y_i) + \lambda  g(\W),
\end{equation}
where $m$ is the number of tasks. The datasets for the tasks are denoted by $\calD^m = (\X^m,\y^m) = \{(\X_1,\y_1),\ldots,(\X_m,\y_m)\}$, where for each $i\in[m]$, $\calD_i = (\X_i,\y_i)$, where $\X_i\in \mathbb{R}^{n_i \times d}$ and $\y_i\in \mathbb{R}^{n_i \times 1} $ denote the data matrix and target vector of the $i$-th task with $n_i$ samples and dimensionality $d$, respectively. $\calL_i$ is the prediction loss function for the $i$-th task. In this paper, we will focus on linear MTL models, where $\w_i$ denotes the model/predictor for task $i$ and
$\W=[\w_1,\w_2,\cdots,\w_m]\in \mathbb{R}^{d \times m}$ is the model parameter matrix. $g(\cdot)$ is a regularization term that represents the structure of the information shared among the tasks, for which $\lambda$ is the pre-fixed hyper-parameter. As a special case, STL can be described by \eqref{eq:MTL_ONE} with $\lambda = 0$.

The key to MTL is to relate the tasks via a shared representation, which, in turn, benefits the tasks to be learned. Each possible shared representation encodes certain assumptions regarding the task relatedness.

{\color{blue}A typical/main-stream assumption is that the tasks share a latent low-rank subspace, as stated by \citet{zhang2017survey} in their survey on MTL, and also by \citet{su2018multi} and \citet{gu2016low}; see, e.g.,~\citet{ando2005framework},~\citet{chen2009convex},~\citet{xu2012conditional},~\citet{han2016multi}, and~\citet{zhen2018multi}.} The formulation leads to a low-rank structure of the model matrix. Because optimization problems involving rank functions are intractable, a trace-norm penalty is typically used~\citep{amit2007uncovering, ji2009accelerated, pong2010trace}, as in the following problem, which will be referred to as the \emph{trace-norm-regularized MTL problem}.
\begin{equation}\label{eq:MTL_Trace}
\min_{\W} \ \sum\nolimits_{i=1}^m\calL_i(\X_i\w_i,\y_i) + \lambda \|\W\|_{*}.
\end{equation}

Another typical assumption is that all tasks share a subset of important features. Such task relatedness can be captured by imposing a group-sparse penalty on the predictor matrix to select shared features across tasks~\citep{turlach2005simultaneous,wright2009sparse,liu2009multi}. One commonly used group-sparse penalty is the group $\ell_1$ penalty~\citep{liu2009multi,nie2010efficient}, as in the following problem, which will be referred to as the \emph{group-$\ell_1$-regularized MTL problem}.
 \begin{equation}\label{eq:MTL_L21}
\min_{\W} \ \sum\nolimits_{i=1}^m\calL_i(\X_i\w_i,\y_i) + \lambda \|\W\|_{2,1}.
\end{equation}


 
Now, we will present a compact definition of the model-protection problem in the context of MTL and discuss the general approach without differential privacy. As can be seen from \eqref{eq:MTL_ONE}, as a result of the joint learning process, $\widehat{\w}_j$ may contain some information on $\widehat{\w}_i$, for $i,j\in[m]$ and $i\neq j$. Then, it is possible for the owner of task $j$ to use such information to attack task $i$. Thus, we define the model-protection problem as follows.
\begin{definition}[Model-Protection Problem for MTL]\label{th:df_MP-MTL_problem}
The model-protection problem for MTL has three objectives:

1) minimizing the information on $\widehat{\w}_i$ that can be inferred from $\widehat{\w}_{[-i]}$, for all $i\in[m]$;

2) maximizing the prediction performance of $\widehat{\w}_i$, for all $i\in[m]$; and

3) sharing useful predictive information among tasks.
\end{definition}

Now, we consider such a procedure: a trusted curator collects independently-trained models, denoted by $\w_1,\ldots,\w_m$, for all tasks \emph{without their associated data} to be used as input. After the joint learning process, the curator outputs the updated models, denoted by $\widehat{\W}$, and sends each updated model to each task privately. The model collection and joint learning processes are performed alternatively.  




%In each iteration, for all $i\in[m]$, the model $\widehat{\w}_i$ updated by the curator is used by the $i$-th task only to generate its independently trained model to be collected for the next iteration.
{
We note that the \emph{trace-norm-regularized MTL problem} and the \emph{group-$\ell_1$-regularized MTL problem} are unified in the multi-task
feature learning framework, which is based on the covariance matrix of the tasks' predictors~\citep{argyriou2007spectral,evgeniou2007multi,argyriou2008convex}. Many other MTL methods also fall under this framework, such as the learning of clustered structures among tasks~\citep{gu2009learning,zhou2011clustered} and the inference of task relations~\citep{zhang2010convex,fei2013structured,bonilla2007multi}. As such, we note that the tasks' covariance matrix constitutes a major source of shared knowledge in MTL methods, and hence, it is regarded as the primary target for model protection.

Therefore, we address the model-protection problem by first rephrasing the first objective in Definition \ref{th:df_MP-MTL_problem} as follows: minimizing the changes in $\widehat{\w}_{[-i]}$ and the tasks' covariance matrix ($\widehat{\W}\widehat{\W}\trans$ or $\widehat{\W}\trans\widehat{\W}$) when task $i$ participates in the joint learning process, for all $i\in[m]$. Thus, the model of this new task is protected.

Then, we find that the concept of differential privacy (minimizing the change in the output distribution) can be adopted to further rephrase this objective as follows: minimizing the changes in \emph{the distribution of} $\widehat{\w}_{[-i]}$ and the tasks' covariance matrix when task $i$ participates in the joint learning process, for all $i\in[m]$.
}

In differential privacy, algorithms are randomized by introducing some kind of perturbation.
\begin{definition}[Randomized Algorithm]\label{th:df_rand_alg}
  {A randomized algorithm} $\mathcal{A}: \calD \rightarrow \theta \in \calC$ is {\color{blue}built by introducing some kind of perturbation into} some mapping $\calD \rightarrow \theta \in \calC$. Algorithm $\mathcal{A}$ outputs $\mathcal{A}(\calD) = \theta$ with a density $p(\mathcal{A}(\calD) = \theta)$ for each $\theta\in \calC$. The probability space is over the perturbation introduced into algorithm $\mathcal{A}$.
   \end{definition}
 %In the following, all the randomized algorithms refer to Definition \ref{th:df_rand_alg}.
 In this paper, $\mathcal{A}$ denotes some randomized machine learning estimator, and $\mbox{\boldmath$\theta$}$ denotes the model parameters that we wish to estimate. Perturbations can be introduced into the original learning system via the (1) input data~\citep{Li2014,BCDKMT07}, (2) model parameters~\citep{chaudhuri2008privacy,Ji2014a}, (3)  objective function~\citep{CMS11,Zhang2012}, or (4) optimization process~\citep{Song2013,wang2015privacy}.

 The formal definition of differential privacy is as follows.

\begin{definition}[\citet{dwork2014algorithmic}]\label{th:df_dp_ori}
  A randomized algorithm $\mathcal{A}$ provides $(\epsilon, \delta) $-differential privacy if, for any two adjacent datasets $\mathcal{D}$ and $\mathcal{D}'$ that differ by a single entry and for any set $\mathcal{S}$,
 \begin{align*}
 \mathbb{P}(\mathcal{A}(\mathcal{D})\in \mathcal{S})
 \leq  \exp(\epsilon)\mathbb{P}(\mathcal{A}(\mathcal{D}')\in \mathcal{S}) + \delta,
 \end{align*}
 where $\mathcal{A}(\mathcal{D})$ and $\mathcal{A}(\mathcal{D}')$ are the outputs of $\mathcal{A}$ on the inputs $\mathcal{D}$ and $ \mathcal{D}' $, respectively.
 \end{definition}

 %Now, let $\mathcal{A}$ be some differentially private machine learning estimator, and let $\mbox{\boldmath$\theta$}$ be the model parameters that we want to estimate. Then, following~\citet{chaudhuri2011differentially}, Definition \ref{th:df_dp_ori} can also be expressed as follows to measure how much privacy  $\mathcal{A}$ can preserve.%\\[-.5em]

%\begin{definition}\label{th:df_dp_new}
% A randomized algorithm $\mathcal{A}(\calB)\in \calC$ provides $(\epsilon,\delta)$ - differential privacy if, for any two adjacent datasets $\mathcal{D}$ and $\mathcal{D}'$, which are inputs of $\mathcal{A}$, that differ by a single data point, any parameter $\ttheta$ that is a solution of $\mathcal{A}$, and some constants $\epsilon,\delta\geq 0$, we have, for any set $\mathcal{S}\subseteq\calC$,
% \begin{align*}
%\bbP(\ttheta \in \calS \mid \calB = \mathcal{D}  )
% \leq  \exp(\epsilon)\bbP(\ttheta \in \calS \mid  \calB = \mathcal{D}' ) + \delta,
% \end{align*}
% where $\bbP(\cdot  \mid \calB = \mathcal{D}  )$ is the conditional probability on $\calC$ induced by the output $\mathcal{A}(\calB)$ given a dataset $\calB = \calD$.
% \end{definition}

The privacy loss pair $(\epsilon,\delta)$ is referred to as the privacy budget/loss and quantifies the privacy risk of algorithm $\mathcal{A}$. The intuition is that it is difficult for a potential attacker to infer whether a certain data point has been changed (or added to the dataset $\mathcal{D}$) based on a change in the output distribution. Consequently, the information of any single data point is protected.


%Note that the defined algorithm $\mathcal{A}$ is randomized; the output parameter $\ttheta$ is a random variable whose distribution is conditioned on the dataset $\mathcal{D}$ or $\mathcal{D}'$. In addition, the privacy loss pair $(\epsilon,\delta)$ is referred to as the privacy budget/loss and quantifies the privacy risk of the algorithm $\mathcal{A}$. The intuition is that it makes it difficult for potential attackers to infer whether a certain data point has been changed (or is added to the dataset $\mathcal{D}$) based on a variation in the conditional distribution. As such, the information of any single data point is protected by the randomized algorithm.

Furthermore, note that differential privacy is defined in terms of application-specific adjacent input databases. In our setting, it is the pair of each task's model and dataset to be treated as the ``single entry'' by Definition \ref{th:df_dp_ori}.

%we let each training dataset represent a set of tasks; each dataset contains the data samples for the corresponding tasks. We say that two of these sets are adjacent if they differ by a single entry, that is, if one task is present in one set but absent in the other.

Several mechanisms exist for introducing a specific type of perturbation. A typical type is calibrated to the sensitivity of the original ``unrandomized'' machine learning estimator $f: \mathcal{D}\rightarrow \ttheta\in \mathbb{R}^d$. The sensitivity of an estimator is defined as the maximum change in its output due to an replacement of any single data instance. %\\[-.5em]

\begin{definition}[\citet{dwork2014algorithmic}]
 The sensitivity of a function $f: \mathcal{D}\rightarrow  \mathbb{R}^d$ is defined as
 \begin{align*}
S(f) = \max_{\mathcal{D},\mathcal{D}'}\|f(\mathcal{D}) -f(\mathcal{D}') \|
 \end{align*}
 for all datasets $\mathcal{D}$ and $\mathcal{D}'$ that differ by at most one instance, where $\|\cdot \|$ {\color{blue} is specified by a particular mechanism. E.g., the Gaussian mechanism~\citep{dwork2014analyze} requires the $\ell_2$ norm, and the Laplace mechanism~\citep{dwork2014algorithmic} requires the $\ell_1$ norm.}
 \end{definition}

The use of additive noise, such as Laplace noise~\citep{dwork2014algorithmic} or Gaussian noise~\citep{dwork2014analyze}, with a standard deviation proportional to $S(f)$ is a common practice for guaranteeing private learning. {\color{blue}In this paper, we adopt the Wishart noise for covariance matrices~\citep{jiang2016wishart}, which is defined as follows.
\begin{definition}[\citet{gupta1999matrix}]
A $d \times d$ random symmetric positive definite matrix $\E$ is said to have a
Wishart distribution $\E\sim W_d(\nu,\V)$ if its probability density function is
\begin{equation*}
  p(\E) = \frac{|\E|^{(\nu-d-1)/2}\exp(-\rm tr(\V^{-1}\E)/2)}{2^{\frac{\nu d}{2}}|\V|^{1/2}\Gamma_d(\nu/2)},
\end{equation*}
where $\nu > d-1$ and $\V$ is a $d \times d$ positive definite matrix.
\end{definition}
}


%The exponential mechanism is another typical type of perturbation method, where sensitivity is not explicitly used, and the perturbation is performed by directly sampling from some distribution related to the conditional density $p(\ttheta \mid \mathcal{D})$~\citep{dwork2014algorithmic,chaudhuri2013near}.

Because machine learning schemes are usually presented as sequential paradigms with multiple iterations and usually output multiple variables simultaneously, several properties of differential privacy are particularly useful for ensuring privacy in machine learning, such as its post-processing immunity, group privacy, composition properties and adaptive composition. The details of these properties are introduced in the supplementary material.


%\section{Wishart Distribution}\label{sec:df_wishart}
%In this paper, the Wishart distribution will be used, which is defined below.


